Censored Quantile Regression Neural Networks for Distribution-Free Survival Analysis

This paper considers doing quantile regression on censored data using neural networks (NNs). This adds to the survival analysis toolkit by allowing direct prediction of the target variable, along with a distribution-free characterisation of uncertainty, using a flexible function approximator. We begin by showing how an algorithm popular in linear models can be applied to NNs. However, the resulting procedure is inefficient, requiring sequential optimisation of an individual NN at each desired quantile. Our major contribution is a novel algorithm that simultaneously optimises a grid of quantiles output by a single NN. To offer theoretical insight into our algorithm, we show firstly that it can be interpreted as a form of expectation-maximisation, and secondly that it exhibits a desirable `self-correcting' property. Experimentally, the algorithm produces quantiles that are better calibrated than existing methods on 10 out of 12 real datasets.

==> QRNN_censored_01(8) copy/NeuRIPS2022/checklist_01.tex <==

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec_discuss_conclude}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{We don't foresee direct negative societal impacts from our algorithm.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix \ref{sec_app_theory}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Code is available at \textcolor{blue}{\url{https://github.com/TeaPearce/Censored_Quantile_Regression_NN}}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix \ref{sec_app_exp_details_hyperparam}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Standard errors over ten random seeds are included in main results in Figure \ref{fig_metric_plots} and Table \ref{tab_full_resultsa}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{sec_app_exp_details}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Data details are given in Appendix \ref{sec_app_dataset_details}.}
  \item Did you mention the license of the assets?
    \answerYes{All datasets used are opensourced.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We don't create new assets. Links to datasets used are provided in Appendix \ref{sec_app_dataset_details}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Data details are given in Appendix \ref{sec_app_dataset_details}.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> QRNN_censored_01(8) copy/tables_figs_etc/algorithm_cqrnn.tex <==
\begin{algorithm}[t]
\caption{CQRNN algorithm.}\label{alg_cqrnn_loss}
\begin{algorithmic}
% \Require Dataset $\mathcal{D}$, parametric model $\psi(\cdot)$ with randomly initialised parameters $\theta_\tau$ for each quantile to estimated, $\operatorname{grid}_\tau$, learning rate $\alpha$, large y value, $y^*$.
\Require Dataset $\mathcal{D}$, one parametric model $\psi(\cdot)$ with randomly initialised parameters $\theta$ that can output $M$ quantile predictions, quantiles to be estimated $\operatorname{grid}_\tau$, learning rate $\alpha$, pseudo y value $y^*$.
\newline
\State $\mathcal{S}_\text{censored} \gets$  $\{i \in \{0,1, \dots , N\} : \Delta_i = 0 \}, \mathcal{S}_\text{observed} \gets$  $\{i \in \{0,1, \dots , N\} : \Delta_i = 1 \}$ %\Comment{Collect indices of censored observations} 
\While{\textbf{not} convereged}
    % \For{\textbf{each} Mini-batch $\mathcal{D}_B \in \mathcal{D}$}
        % \State $\text{censored}_B \gets$  $\{i \in \mathcal{D}_B : \Delta_i = 0 \}$\Comment{Collect indices of censored observations}
        % \State $\text{observed}_B \gets$  $\{i \in \mathcal{D}_B : \Delta_i = 1 \}$
        % \For{$j \in \text{censored}_B$}
        \State \textit{1. Hard expectation step}
        \For{$j \in \mathcal{S}_\text{censored}$} %\Comment{1. Expectation step}
        \State $\hat{q}_j \gets \arg \min_\tau |\hat{y}_{j,\tau} -  y_j|$ \Comment{Estimate quantile of censored data under current model}
        \State $\hat{w}_j \gets (\tau - \hat{q}_j)/(1 - \hat{q}_j)$
        \EndFor
        \State \textit{2. Partial maximisation step}
        % \For{$\tau \in \text{grid}_\tau$} \Comment{Can be parallelised}
        \State $\theta \gets \theta - \alpha \partial\mathcal{L}(\theta_\tau, \mathcal{D}, \tau, \mathbf{\hat{w}}, y^*) / \partial \theta \;\; \forall \tau \in \operatorname{grid}_\tau$ \Comment{Gradient step to minimise Eq. \ref{eq_loss_reweight}} %, optionally add $\mathcal{L}_\text{cross}$}
        % \EndFor
    % \EndFor
\EndWhile
\end{algorithmic}
\end{algorithm}

==> QRNN_censored_01(8) copy/tables_figs_etc/algorithm_seqgrid.tex <==
\begin{algorithm}[t]
\caption{Sequential grid algorithm for NNs.}\label{alg_seq_grid}
\begin{algorithmic}
\Require Dataset $\mathcal{D}$, $M$ parametric models $\psi_\tau(\cdot)$ each with randomly initialised parameters $\theta_\tau$, ordered quantiles to be estimated $\operatorname{grid}_\tau$, learning rate $\alpha$, pseudo y value $y^*$.
\newline
\State $\mathcal{S}_\text{censored} \gets$  $\{i \in \{0,1, \dots , N\} : \Delta_i = 0 \}, \mathcal{S}_\text{observed} \gets$  $\{i \in \{0,1, \dots , N\} : \Delta_i = 1 \}$, $K_\text{cross} \gets \emptyset $

%\Comment{Collect indices of censored observations} 
% \While{\textbf{not} convereged}
% \For{$\tau \in \operatorname{grid}_\tau$}
\For{$i = 0$ \textbf{to} $M-1$}
    % \For{\textbf{each} Mini-batch $\mathcal{D}_B \in \mathcal{D}$}
        \State $\tau \gets \operatorname{grid}_\tau[i]$
        % \State $\text{censored}_B \gets$  $\{i \in \mathcal{D}_B : \Delta_i = 0 \}$\Comment{Collect indices of censored observations}
        % \State $\text{observed}_B \gets$  $\{i \in \mathcal{D}_B : \Delta_i = 1 \}$
        % \For{$j \in \text{censored}_B$}
        % \State \textit{1. Hard expectation step}
        % \If {$\tau = min_\tau \operatorname{grid}_\tau$}
        \If {$i = 0$} \Comment{Initialise quantile estimates to zero}
        \State $\mathbf{\hat{q}} \gets \operatorname{zeros(N_c)}$ 
        % \Comment{The exact value has no effect until the censored datapoint is crossed, at which point it is updated anyway}
        \Else \Comment{Find indices which have been crossed and update their estimated quantiles}
        \State $K \gets \{ j \in \mathcal{S}_\text{censored}: \psi_{\operatorname{grid}_\tau[i-1]}(\x_j) \leq y_j \cap \psi_{\operatorname{grid}_\tau[i]}(\x_j) >  y_j \}$ 
        \State $\mathbf{\hat{q}}[K] \gets  \operatorname{grid}_\tau[i-1]$
        \State $K_\text{cross} \gets K_\text{cross} \cup K$ %, \;\; \mathbf{\hat{q}}[\neg K_\text{cross}] \gets \tau$ \Comment{Sets $\mathbf{w}=0$  for uncrossed datapoints}
        \State $\mathbf{\hat{q}}[\neg K_\text{cross}] \gets \tau$ \Comment{Sets $\mathbf{\hat{w}}=0$  for uncrossed datapoints}
        % \State $\mathbf{w}[K] \gets (\tau - \hat{q}_j)/(1 - \hat{q}_j) \operatorname{grid}_\tau[i-1]$
        % \Else
        % asdf
        % \ElsIf{asdf}
        % sadf
        % \State \tp{I think need to check if all datapoints crossed, then exit}
        \EndIf
        
        \State $\mathbf{\hat{w}} \gets (\tau - \mathbf{\hat{q}})/(1 - \mathbf{\hat{q}})$
        
        \State $\theta \gets \arg \min_{\theta_\tau} \mathcal{L}_\text{Port.}(\theta_\tau, \mathcal{D}, \tau, \mathbf{\hat{w}}, y^*) $  \Comment{Fully optimise Eq. \ref{eq_loss_reweight}}
        
        % \Comment{Fully optimise eq. \ref{eq_loss_reweight}}
        % \While{\textbf{not} convereged}  
        % \State $\theta \gets \theta - \alpha \partial\mathcal{L}(\theta_\tau, \mathcal{D}, \tau, \mathbf{w}, y^*) / \partial \theta$ 
        % \EndWhile
        
        % \For{$j \in \mathcal{S}_\text{censored}$} %\Comment{1. Expectation step}
        % \State $\hat{q}_j \gets \arg \min_\tau |\hat{y}_{j,\tau} -  y_j|$ \Comment{Estimate quantile of censored data under current model}
        % \State $w_j \gets (\tau - \hat{q}_j)/(1 - \hat{q}_j)$
        % \EndFor
        % \State \textit{2. Partial maximisation step}
        % \For{$\tau \in \text{grid}_\tau$} %\Comment{2. Partial maximisation step}
        
        % \EndFor
    % \EndFor
% \EndWhile
\EndFor
\end{algorithmic}
\end{algorithm}
% \vspace{-0.5in}

==> QRNN_censored_01(8) copy/tables_figs_etc/fig_1D_02.tex <==
\begin{figure}[h!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

\small CQRNN (ours) \hspace{0.6in}  Excl. censor \hspace{0.6in}  DeepQuantReg \hspace{0.6in}  LogNorm MLE


\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_cqrnn_v01.pdf}
\put(-107,2){\rotatebox{90}{\small Norm1D uniform}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_lognorm_v01.pdf}
\put(-0,4){\transparent{1.}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}
% \put(-42,4){\transparent{0.9}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}


\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_cqrnn_v01.pdf}
\put(-107,7){\rotatebox{90}{\small Norm1D linear}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_lognorm_v01.pdf}

\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_cqrnn_v01.pdf}
\put(-107,5){\rotatebox{90}{\small Norm1D non-lin.}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_lognorm_v01.pdf}


\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_cqrnn_v01.pdf}
\put(-107,8){\rotatebox{90}{\small Exponential1D}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_lognorm_v01.pdf}

\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_cqrnn_v01.pdf}
\put(-107,18){\rotatebox{90}{\small Weibull1D}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_lognorm_v01.pdf}

\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_cqrnn_v01.pdf}
\put(-107,10){\rotatebox{90}{\small LogNorm1D}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_lognorm_v01.pdf}





\caption{This figure shows estimated quantiles (blue through pink) compared to ground truth quantiles (dashed black lines).
It shows 1D synthetic datasets of varying functions and noise distributions (rows), fitted by various methods (columns).
% described in table \ref{tab_dataset_info}
CQRNN recovers quantiles closest to the ground truth on most datasets.}
\label{fig_1D_plots}
\end{center}
\vskip -0.2in
\end{figure}

==> QRNN_censored_01(8) copy/tables_figs_etc/fig_1D_02_grid.tex <==
\begin{figure}[h!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

\hspace{0.2in} \small CQRNN   \hspace{0.4in}  Sequential grid  \hspace{0.4in}  Excl. censor \hspace{0.4in}  DeepQuantReg \hspace{0.35in}  LogNorm MLE


\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_cqrnn_v01.pdf}
\put(-85,0){\rotatebox{90}{\small Norm uniform}}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_neocleous_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_excl_censor_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_deepquantreg_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_lognorm_v01.pdf}
\put(-0,4){\transparent{1.}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}
% \put(-42,4){\transparent{0.9}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}


\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_cqrnn_v01.pdf}
\put(-85,0){\rotatebox{90}{\small Norm linear}}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_neocleous_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_excl_censor_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_deepquantreg_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_lognorm_v01.pdf}

\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_cqrnn_v01.pdf}
\put(-85,0){\rotatebox{90}{\small Norm non-lin.}}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_neocleous_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_excl_censor_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_deepquantreg_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_lognorm_v01.pdf}


\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Exponential_cqrnn_v01.pdf}
\put(-85,0){\rotatebox{90}{\small Exponential}}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Exponential_excl_censor_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Exponential_deepquantreg_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Exponential_lognorm_v01.pdf}

\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Weibull_cqrnn_v01.pdf}
\put(-85,0){\rotatebox{90}{\small Weibull}}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Weibull_neocleous_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Weibull_excl_censor_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Weibull_deepquantreg_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_Weibull_lognorm_v01.pdf}

\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_LogNorm_cqrnn_v01.pdf}
\put(-85,0){\rotatebox{90}{\small LogNorm}}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_LogNorm_neocleous_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_LogNorm_excl_censor_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_LogNorm_deepquantreg_v01.pdf}
\includegraphics[width=0.195\columnwidth]{images/1D_plots/1Dinput_LogNorm_lognorm_v01.pdf}



\caption{This figure shows estimated quantiles (blue through pink) compared to ground truth quantiles (dashed black lines).
It shows 1D synthetic datasets of varying functions and noise distributions (rows), fitted by various methods (columns).
% described in table \ref{tab_dataset_info}
% CQRNN recovers quantiles closest to the ground truth on most datasets.
}
\label{fig_1D_plots}
\end{center}
\vskip -0.2in
\end{figure}

==> QRNN_censored_01(8) copy/tables_figs_etc/fig_1D_mini_01.tex <==
\begin{figure}[b!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

\small CQRNN (ours) \hspace{0.6in}  Excl. censor \hspace{0.6in}  DeepQuantReg \hspace{0.6in}  LogNorm MLE

\vspace{-0.05in}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_cqrnn_v01.pdf}
\put(-107,0){\rotatebox{90}{\small Norm uniform}}
% \put(-107,5){\rotatebox{90}{\small uniform}}
% \put(-117,5){\rotatebox{90}{\small Norm1D}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_lognorm_v01.pdf}
\put(-0,4){\transparent{1.}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}
% \put(-42,4){\transparent{0.9}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}


\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_cqrnn_v01.pdf}
\put(-107,4){\rotatebox{90}{\small Norm linear}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_lognorm_v01.pdf}

% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_cqrnn_v01.pdf}
% \put(-107,5){\rotatebox{90}{\small Norm1D non-lin.}}
% % \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_neocleous_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_excl_censor_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_deepquantreg_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_lognorm_v01.pdf}


\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_cqrnn_v01.pdf}
\put(-107,8){\rotatebox{90}{\small Exponential}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_lognorm_v01.pdf}

% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_cqrnn_v01.pdf}
% \put(-107,18){\rotatebox{90}{\small Weibull1D}}
% % \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_excl_censor_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_deepquantreg_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_lognorm_v01.pdf}

\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_LogNorm_cqrnn_v01.pdf}
\put(-107,6){\rotatebox{90}{\small LogNorm}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_LogNorm_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_LogNorm_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth,height=0.13\columnwidth]{images/1D_plots/1Dinput_LogNorm_lognorm_v01.pdf}





\caption{1D synthetic datasets of varying functions (rows), fitted by various methods (columns). Estimated quantiles (blue through pink) compared to ground truth quantiles (dashed black lines).
CQRNN recovers quantiles closest to the ground truth on most datasets.}
\label{fig_1D_plots_mini}
\end{center}
\vskip -0.2in
\end{figure}

==> QRNN_censored_01(8) copy/tables_figs_etc/fig_bench_cindex_dcal_02.tex <==
\begin{figure}[t!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_legend_synth_1D_test_q_metric_selected_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_ND_test_q_metric_selected_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_cens_test_quantile_sum_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_cens_test_Dcal_nocens_v01.pdf}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_1D_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_1D_test_cens_Dcal_cens_v01.pdf}
\put(-0,15){\transparent{1.}\includegraphics[width=0.1\columnwidth]{images/main_results/mainresults_legend_01.pdf}}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_ND_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_ND_test_cens_Dcal_cens_v01.pdf}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_cens_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_cens_test_cens_Dcal_cens_v01.pdf}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_real_cens_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_real_cens_test_cens_Dcal_cens_v01.pdf}

\caption{Main results. Mean $\pm$ one standard error over ten runs. See table \ref{tab_full_results} for further assessed metrics.}
\label{fig_metric_plots_cindex_dcal}
\end{center}
\vskip -0.2in
\end{figure}

==> QRNN_censored_01(8) copy/tables_figs_etc/fig_bench_main_01.tex <==
% main benchmarking figures, with metrics selected per dataset

% \begin{figure}[t!]
\begin{wrapfigure}{R}{0.5\textwidth} 
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.4in}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_legend_synth_1D_test_q_metric_selected_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_ND_test_q_metric_selected_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_cens_test_quantile_sum_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_cens_test_Dcal_nocens_v01.pdf}

Type 1 datasets 
% -- Synthetic data with  synthetic censoring

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_1D_test_q_metric_selected_v01.pdf}
\put(-0,8){\transparent{1.}\includegraphics[width=0.13\columnwidth]{images/main_results/mainresults_legend_01.pdf}}

% Type 1 -- Multidimensional datasets

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_ND_test_q_metric_selected_v01.pdf}




% \includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_ND_test_cens_cindex_median_v01.pdf}
% \includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_ND_test_cens_Dcal_cens_v01.pdf}
Type 2 datasets
% -- Real datasets with synthetic censoring

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_cens_test_quantile_sum_v01.pdf}
% \includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_cens_test_cens_Dcal_cens_v01.pdf}

Type 3 datasets
% -- Real datasets with real censoring

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_real_cens_test_cens_cindex_median_v01.pdf}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_real_cens_test_cens_Dcal_cens_v01.pdf}

\caption{Main benchmarking results. Mean $\pm$ one standard error over ten runs.} 
% See table \ref{tab_full_results} for further assessed metrics.}
\label{fig_metric_plots}
\end{center}
\vskip -0.6in
% \end{figure}
\end{wrapfigure}

==> QRNN_censored_01(8) copy/tables_figs_etc/fig_grid_ablation_01.tex <==
\begin{figure}[b!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

% \small CQRNN (ours) \hspace{0.6in}  Excl. censor \hspace{0.6in}  DeepQuantReg \hspace{0.6in}  LogNorm MLE


\hspace{0.45in} Norm linear \hspace{0.45in} Norm uniform \hspace{0.45in} Norm non-linear

\includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_Gaussian_linear_test_q_metric_selected_v01.pdf}
% \put(-107,2){\rotatebox{90}{\small Normal uniform}}
\includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_Gaussian_uniform_test_q_metric_selected_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_Exponential_test_q_metric_selected_v01.pdf}
\put(-0,50){\transparent{1.}\includegraphics[width=0.15\columnwidth]{images/grid_ablation/converge_legend_01.pdf}}

\hspace{0.3in} Exponential \hspace{0.7in} Weibull \hspace{0.7in} LogNorm


\includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_Gaussian_nonlinear_test_q_metric_selected_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_Weibull_test_q_metric_selected_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_LogNorm_test_q_metric_selected_v01.pdf}

% \hspace{0.35in} Normal4D light \hspace{0.35in} Normal4D medium \hspace{0.35in} Normal4D heavy

% \includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_GaussianUniform4D_v1_light_test_q_metric_selected_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_Gaussian_Uniform4D_v1_test_q_metric_selected_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_GaussianUniform4D_v1_heavy_test_q_metric_selected_v01.pdf}

% \hspace{0.35in} LogNormal8D Light \hspace{0.35in} LogNormal8D Medium \hspace{0.35in} LogNormal8D Heavy

% \includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_LogNorm_v1_light_test_q_metric_selected_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_LogNorm_v1_test_q_metric_selected_v01.pdf}
% \includegraphics[width=0.245\columnwidth]{images/grid_ablation/converge_LogNorm_v1_heavy_test_q_metric_selected_v01.pdf}







\caption{Ablations over grid size and number of datapoints for various synthetic datasets using our CQRNN method.}
% Note that MSE between predicted and ground truth quantiles decreases under increasing dataset size. A larger grid size tends to produce lower MSE, and this is particularly important in datasets with uniform censoring. But this is not always the case; notably for small datasets, a larger grid can be slightly harmful for datasets with non-uniform censoring.}
\label{fig_grid_ablation}
\end{center}
\vskip -0.2in
\end{figure}

==> QRNN_censored_01(8) copy/tables_figs_etc/fig_partial_full_01.tex <==
\begin{figure}[h!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

% \hspace{0.2in} \small CQRNN   \hspace{0.4in}  Sequential grid  \hspace{0.4in}  Excl. censor \hspace{0.4in}  DeepQuantReg \hspace{0.35in}  LogNorm MLE

\includegraphics[width=0.32\columnwidth]{images/partial_full/partial_vs_full_NormLinear_cqrnn.pdf}
% \put(-85,0){\rotatebox{90}{\small Norm uniform}}
\includegraphics[width=0.32\columnwidth]{images/partial_full/partial_vs_full_NormLinear_fullopt1.pdf}
\includegraphics[width=0.32\columnwidth]{images/partial_full/partial_vs_full_NormLinear_fullopt10.pdf}
\includegraphics[width=0.32\columnwidth]{images/partial_full/partial_vs_full_NormLinear_fullopt25.pdf}
\includegraphics[width=0.32\columnwidth]{images/partial_full/partial_vs_full_NormLinear_fullopt50.pdf}
\includegraphics[width=0.32\columnwidth]{images/partial_full/partial_vs_full_NormLinear_fullopt100.pdf}

% \put(-42,4){\transparent{0.9}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}

\caption{This figure explores the effect of optimising the NNs partially compared to fully. It shows training loss and TQMSE over training epochs. The Normal Linear dataset was used. 
% Observe that partial maximisation, using the most up-to-date estimates of $\hat{q}_i$, converges quicker than when only updating $\hat{q}_i$ after a certain number of epochs. A longer time between updates delays convergence.
}
\label{fig_partial_full}
\end{center}
\vskip -0.2in
\end{figure}

==> QRNN_censored_01(8) copy/tables_figs_etc/table_comparison_grid_01.tex <==
\begin{table}[ht]
\centering
\resizebox{1.\textwidth}{!}{\begin{tabular}{lrrrrrrr}

\toprule
%   dataset\_str &  diff\_time\_training\_time &  diff\_time\_test\_fwdpass\_time &  diff\_test\_q\_metric\_selected &  diff\_test\_quantile\_sum &  diff\_test\_cens\_cindex\_median &  time\_training\_time &  diff\_test\_cens\_Dcal\_cens \\
    & & \multicolumn{6}{c}{---------------------------------------------- Difference: CQRNN - Sequential-grid ----------------------------------------------}\\ 
    
    
   Dataset &  Number & Training time (seconds) &  Test time (seconds) &  TQMSE &  Uncensored quantile loss  &  Concordance-Index &  Censored D-Calibration \\
   
    & quantiles & (lower better) &  (lower better) & (lower better) &  (lower better)  &  (higher better) &  (lower better) \\
   
%   Uncensored quantile loss & Uncensored D-Calibration & Concordance-Index & Censored D-Calibration

\midrule
   Norm linear &           10 &                   -4.997 &                       -0.015 &                       -2.691 &                  -0.106 &                         0.001 &                    -0.013 \\
  Norm non-lin &           10 &                   -5.336 &                       -0.017 &                        0.001 &                   0.000 &                         0.001 &                    -0.008 \\
   Exponential &           10 &                   -7.528 &                       -0.026 &                       -0.404 &                  -0.004 &                         0.001 &                     0.022 \\
       Weibull &           10 &                   -7.274 &                       -0.023 &                       -0.006 &                   0.002 &                         0.000 &                     0.002 \\
       LogNorm &           10 &                   -6.145 &                       -0.018 &                        0.083 &                   0.000 &                        -0.001 &                    -0.032 \\
  Norm uniform &           10 &                   -4.853 &                       -0.015 &                        0.200 &                   0.033 &                         0.001 &                    -0.368 \\
    Norm heavy &           20 &                  -23.801 &                       -0.097 &                       -0.018 &                   0.003 &                        -0.001 &                     0.103 \\
     Norm med. &           20 &                  -24.384 &                       -0.102 &                       -0.050 &                  -0.010 &                         0.001 &                    -0.002 \\
    Norm light &           20 &                  -24.417 &                       -0.097 &                       -0.038 &                  -0.006 &                         0.000 &                    -0.106 \\
     Norm same &           20 &                  -29.910 &                       -0.125 &                       -0.685 &                  -0.062 &                         0.002 &                    -0.050 \\
 LogNorm heavy &           20 &                  -45.441 &                       -0.268 &                        0.004 &                   0.002 &                         0.001 &                    -0.008 \\
  LogNorm med. &           20 &                  -33.679 &                       -0.195 &                        0.014 &                   0.002 &                         0.000 &                    -0.034 \\
 LogNorm light &           20 &                  -45.157 &                       -0.248 &                       -0.026 &                  -0.003 &                         0.000 &                    -0.075 \\
  LogNorm same &           20 &                  -27.471 &                       -0.158 &                       -0.285 &                  -0.018 &                        -0.001 &                    -0.046 \\

\midrule
Datasets where  & & 14/14 & 14/14 & 9/14 & 8/14 & 9/14 & 11/14 \\
CQRNN is favoured  \\
\bottomrule



\end{tabular}}
\label{tab_grid_cqrnn_compare}
\caption{Performance comparison of our proposed CQRNN algorithm (alg. \ref{alg_cqrnn_loss}) with the sequential grid-based method from \cite{Neocleous2006}, which we've adapted for neural networks.
% Both optimise Portnoy's estimator, but 
For all quantile metrics CQRNN has a slight advantage (e.g. wins on 9/14 datasets in MSE). Running time for the sequential grid is significantly slower at both train and test time (and also in memory requirements). This arises from its running time scaling with, $\mathcal{O}(\text{no. quantiles})$. \tp{could delete other metric columns, keep TQMSE and put inline w text? Need parameter count}}
\end{table}

==> QRNN_censored_01(8) copy/tables_figs_etc/table_comparison_grid_02.tex <==
\begin{table}[t]
\centering
\caption{Performance of our proposed CQRNN algorithm (algorithm \ref{alg_cqrnn_loss}) compared to the sequential grid method for NNs (algorithm \ref{alg_seq_grid}). All datasets shown -- extended version of table \ref{tab_grid_cqrnn_compare_mini}.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}
\resizebox{0.7\textwidth}{!}{\begin{tabular}{lrrrrrrr}

\toprule
   Dataset &  Number & Training time &  Test time &  Parameter & TQMSE difference  \\
  
    & quantiles & speed up &  speed up & saving &  Seq. grid $-$ CQRNN  \\
    % &&&&& Seq. grid $-$ CQRNN\\
%   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\
\midrule
   Norm linear &           10 &                    14.7$\times$ &                        11.2$\times$ &             9.2$\times$ &                         -2.691 \\
  Norm non-lin &           10 &                    12.4$\times$ &                         9.6$\times$ &             9.2$\times$ &                          0.001 \\
   Exponential &           10 &                    12.4$\times$ &                         8.0$\times$ &             9.2$\times$ &                         -0.404 \\
       Weibull &           10 &                    12.5$\times$ &                         8.7$\times$ &             9.2$\times$ &                         -0.006 \\
       LogNorm &           10 &                    12.9$\times$ &                         8.8$\times$ &             9.2$\times$ &                          0.083 \\
  Norm uniform &           10 &                    12.6$\times$ &                         8.1$\times$ &             9.2$\times$ &                          0.200 \\
    Norm heavy &           20 &                    31.0$\times$ &                        18.5$\times$ &             17.1$\times$ &                         -0.018 \\
     Norm med. &           20 &                    34.1$\times$ &                        17.9$\times$ &             17.1$\times$ &                         -0.050 \\
    Norm light &           20 &                    31.7$\times$ &                        19.2$\times$ &             17.1$\times$ &                         -0.038 \\
     Norm same &           20 &                    34.3$\times$ &                        21.2$\times$ &             17.1$\times$ &                         -0.685 \\
 LogNorm heavy &           20 &                    33.6$\times$ &                        19.9$\times$ &             17.1$\times$ &                          0.004 \\
  LogNorm med. &           20 &                    31.3$\times$ &                        13.1$\times$ &             17.1$\times$ &                          0.014 \\
 LogNorm light &           20 &                    31.3$\times$ &                        20.2$\times$ &             17.1$\times$ &                         -0.026 \\
  LogNorm same &           20 &                    29.8$\times$ &                        18.4$\times$ &             17.1$\times$ &                         -0.285 \\
\midrule
CQRNN is best:   & & 14/14 & 14/14 & 14/14 & 9/14 \\
% CQRNN is best  \\
\bottomrule

\end{tabular}}
\label{tab_grid_cqrnn_compare}
\end{table}

==> QRNN_censored_01(8) copy/tables_figs_etc/table_comparison_grid_02_mini.tex <==
\begin{table}[t]
\centering
\caption{Performance of our proposed CQRNN algorithm (Algorithm \ref{alg_cqrnn_loss}) compared to the sequential grid method for NNs (Algorithm \ref{alg_seq_grid}). Select datsets shown -- see Table \ref{tab_grid_cqrnn_compare} for others.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}
\resizebox{0.6\textwidth}{!}{\begin{tabular}{lrrrrrrr}

\toprule
   Dataset &  Number & Training time &  Test time &  Parameter & TQMSE  \\
  
    & quantiles & speed up &  speed up & saving &  difference  \\
%   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\
\midrule
%   Norm linear &           10 &                    14.7$\times$ &                        11.2$\times$ &             9.2$\times$ &                         -2.691 \\
  Norm non-linear &           10 &                    12.4$\times$ &                         9.6$\times$ &             9.2$\times$ &                          0.001 \\
  Exponential &           10 &                    12.4$\times$ &                         8.0$\times$ &             9.2$\times$ &                         -0.404 \\
      Weibull &           10 &                    12.5$\times$ &                         8.7$\times$ &             9.2$\times$ &                         -0.006 \\
    %   LogNorm &           10 &                    12.9$\times$ &                         8.8$\times$ &             9.2$\times$ &                          0.083 \\
%   Norm uniform &           10 &                    12.6$\times$ &                         8.1$\times$ &             9.2$\times$ &                          0.200 \\
    % Norm heavy &           20 &                    31.0$\times$ &                        18.5$\times$ &             17.1$\times$ &                         -0.018 \\
    %  Norm med. &           20 &                    34.1$\times$ &                        17.9$\times$ &             17.1$\times$ &                         -0.050 \\
    % Norm light &           20 &                    31.7$\times$ &                        19.2$\times$ &             17.1$\times$ &                         -0.038 \\
    %  Norm same &           20 &                    34.3$\times$ &                        21.2$\times$ &             17.1$\times$ &                         -0.685 \\
 LogNorm heavy &           20 &                    33.6$\times$ &                        19.9$\times$ &             17.1$\times$ &                          0.004 \\
%   LogNorm med. &           20 &                    31.3$\times$ &                        13.1$\times$ &             17.1$\times$ &                          0.014 \\
 LogNorm light &           20 &                    31.3$\times$ &                        20.2$\times$ &             17.1$\times$ &                         -0.026 \\
%   LogNorm same &           20 &                    29.8$\times$ &                        18.4$\times$ &             17.1$\times$ &                         -0.285 \\
% \midrule
% CQRNN is best:   & & 14/14 & 14/14 & 14/14 & 9/14 \\
% CQRNN is best  \\
\bottomrule

\end{tabular}}
\label{tab_grid_cqrnn_compare_mini}
\end{table}

==> QRNN_censored_01(8) copy/tables_figs_etc/table_comparison_grid_03.tex <==
\begin{table}[t]
\centering
\caption{Performance of our proposed CQRNN algorithm (Algorithm \ref{alg_cqrnn_loss}) compared to the sequential grid method for NNs (Algorithm \ref{alg_seq_grid}), over 200 random seeds.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{lrrrrrrrccc}

\toprule
   Dataset &  Number & Training time &  Test time &  Parameter & TQMSE difference  & CQRNN is & Seq. grid is & No statistical \\
  
    & quantiles & speed up &  speed up & saving &  Seq. grid $-$ CQRNN &  sig. better & sig. better & significant \\
    & & & & & 95\% conf. interval & in TQMSE? & in TQMSE? & difference \\
    % &&&&& Seq. grid $-$ CQRNN\\
%   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\
% \midrule
%   Norm linear &           9 &   7.9$\times$ &   6.5$\times$ &  8.3$\times$ &          -2.189 $\pm$ 0.245 & \checkmark & & \\
%  Norm non-lin &           9 &   8.1$\times$ &   6.4$\times$ &  8.3$\times$ &         -0.003 $\pm$ 0.001 & \checkmark & & \\
%   Exponential &           9 &   8.1$\times$ &   6.7$\times$ &  8.3$\times$ &           -0.093 $\pm$ 0.176 &  & & \checkmark\\
%       Weibull &           9 &   8.0$\times$ &   6.6$\times$ &  8.3$\times$ &         -0.014 $\pm$ 0.016 &  & & \checkmark \\
%       LogNorm &           9 &   8.2$\times$ &   6.8$\times$ &  8.3$\times$ &         -0.039 $\pm$ 0.028 & \checkmark & & \\
%  Norm uniform &           9 &   8.2$\times$ &   6.8$\times$ &  8.3$\times$ &          0.175 $\pm$ 0.033 & & \checkmark  & \\
%   Norm heavy &           19 &  16.2$\times$ &        13.6$\times$ &        16.2$\times$ &           0.108 $\pm$ 0.211 & & & \checkmark\\
%     Norm med. &           19 &  15.4$\times$ &        10.2$\times$ &        16.2$\times$ &          -0.046 $\pm$ 0.004 & \checkmark & & \\
%   Norm light &           19 &  16.2$\times$ &            9.8$\times$ &     16.2$\times$ &         -0.035 $\pm$ 0.003 & \checkmark & & \\
%     Norm same &           19 &  15.8$\times$ &            8.9$\times$ &     16.2$\times$ &         -0.390 $\pm$ 0.049 & \checkmark & & \\
% LogNorm heavy &           19 &  16.0$\times$ &        12.7$\times$ &        16.2$\times$ &          0.005 $\pm$ 0.001 & & \checkmark &  \\
%  LogNorm med. &           19 &  16.6$\times$ &        18.3$\times$ &        16.2$\times$ &          0.019 $\pm$ 0.002 & & \checkmark &  \\
% LogNorm light &           19 &  16.3$\times$ &        15.9$\times$ &        16.2$\times$ &         -0.033 $\pm$ 0.004 & \checkmark & & \\
%  LogNorm same &           19 &  15.8$\times$ &        11.3$\times$ &        16.2$\times$ &         -0.371 $\pm$ 0.045 & \checkmark & & \\
\midrule
  Norm linear &           9 &   14.7$\times$ &   11.2$\times$ &  8.3$\times$ &          -2.189 $\pm$ 0.245 & \checkmark & & \\
 Norm non-lin &           9 &   12.4$\times$ &   9.6$\times$ &  8.3$\times$ &         -0.003 $\pm$ 0.001 & \checkmark & & \\
  Exponential &           9 &   12.4$\times$ &   8.0$\times$ &  8.3$\times$ &           -0.093 $\pm$ 0.176 &  & & \checkmark\\
      Weibull &           9 &   12.5$\times$ &   8.7$\times$ &  8.3$\times$ &         -0.014 $\pm$ 0.016 &  & & \checkmark \\
      LogNorm &           9 &   12.9$\times$ &   8.8$\times$ &  8.3$\times$ &         -0.039 $\pm$ 0.028 & \checkmark & & \\
 Norm uniform &           9 &   12.6$\times$ &   8.1$\times$ &  8.3$\times$ &          0.175 $\pm$ 0.033 & & \checkmark  & \\
   Norm heavy &           19 &  31.0$\times$ &        18.5$\times$ &        16.2$\times$ &           0.108 $\pm$ 0.211 & & & \checkmark\\
    Norm med. &           19 &  34.1$\times$ &        17.9$\times$ &        16.2$\times$ &          -0.046 $\pm$ 0.004 & \checkmark & & \\
   Norm light &           19 &  31.7$\times$ &            19.2$\times$ &     16.2$\times$ &         -0.035 $\pm$ 0.003 & \checkmark & & \\
    Norm same &           19 &  34.3$\times$ &            21.2$\times$ &     16.2$\times$ &         -0.390 $\pm$ 0.049 & \checkmark & & \\
LogNorm heavy &           19 &  33.6$\times$ &        19.9$\times$ &        16.2$\times$ &          0.005 $\pm$ 0.001 & & \checkmark &  \\
 LogNorm med. &           19 &  31.3$\times$ &        13.1$\times$ &        16.2$\times$ &          0.019 $\pm$ 0.002 & & \checkmark &  \\
LogNorm light &           19 &  31.3$\times$ &        20.2$\times$ &        16.2$\times$ &         -0.033 $\pm$ 0.004 & \checkmark & & \\
 LogNorm same &           19 &  29.8$\times$ &        18.4$\times$ &        16.2$\times$ &         -0.371 $\pm$ 0.045 & \checkmark & & \\
% \midrule
\midrule
% CQRNN is best:   & & 14/14 & 14/14 & 14/14 & \\
 Total: & & & & & & 8/14 & 3/14 & 3/14 \\
% CQRNN is best  \\
% \midrule
%   $^*$Norm uniform w/ $M=19$ &           19 &                  15.4 &                       9.3$\times$ &           16.2$\times$ &          0.004 $\pm$ 0.012 & & & \checkmark \\
\bottomrule

\end{tabular}}
\label{tab_grid_cqrnn_compare}
\end{table}

==> QRNN_censored_01(8) copy/tables_figs_etc/table_comparison_grid_03_mini.tex <==
\begin{table}[t]
\centering
\caption{Performance of our proposed CQRNN algorithm compared to the sequential grid method for NNs. See Table \ref{tab_grid_cqrnn_compare} for results on further datasets, as well as statistical significance tests.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}
% \resizebox{0.6\textwidth}{!}{\begin{tabular}{lrrrrrrr}

% \toprule
% %   Dataset &  Number & Training time &  Test time &  Parameter & TQMSE  \\
  
%     % & quantiles & speed up &  speed up & saving &  difference  \\
% %   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\
% \midrule
% %   Norm linear &           10 &                    14.7$\times$ &                        11.2$\times$ &             9.2$\times$ &                         -2.691 \\
%   Norm non-linear &           10 &                    12.4$\times$ &                         9.6$\times$ &             9.2$\times$ &                          0.001 \\
%   Exponential &           10 &                    12.4$\times$ &                         8.0$\times$ &             9.2$\times$ &                         -0.404 \\
%       Weibull &           10 &                    12.5$\times$ &                         8.7$\times$ &             9.2$\times$ &                         -0.006 \\
%     %   LogNorm &           10 &                    12.9$\times$ &                         8.8$\times$ &             9.2$\times$ &                          0.083 \\
% %   Norm uniform &           10 &                    12.6$\times$ &                         8.1$\times$ &             9.2$\times$ &                          0.200 \\
%     % Norm heavy &           20 &                    31.0$\times$ &                        18.5$\times$ &             17.1$\times$ &                         -0.018 \\
%     %  Norm med. &           20 &                    34.1$\times$ &                        17.9$\times$ &             17.1$\times$ &                         -0.050 \\
%     % Norm light &           20 &                    31.7$\times$ &                        19.2$\times$ &             17.1$\times$ &                         -0.038 \\
%     %  Norm same &           20 &                    34.3$\times$ &                        21.2$\times$ &             17.1$\times$ &                         -0.685 \\
%  LogNorm heavy &           20 &                    33.6$\times$ &                        19.9$\times$ &             17.1$\times$ &                          0.004 \\
% %   LogNorm med. &           20 &                    31.3$\times$ &                        13.1$\times$ &             17.1$\times$ &                          0.014 \\
%  LogNorm light &           20 &                    31.3$\times$ &                        20.2$\times$ &             17.1$\times$ &                         -0.026 \\
% %   LogNorm same &           20 &                    29.8$\times$ &                        18.4$\times$ &             17.1$\times$ &                         -0.285 \\
% % \midrule
% % CQRNN is best:   & & 14/14 & 14/14 & 14/14 & 9/14 \\
% % CQRNN is best  \\

\resizebox{0.7\textwidth}{!}{\begin{tabular}{lrrrrrrrccc}

\toprule
   Dataset &  Number & Training time &  Test time &  Parameter  & TQMSE difference \\%  & CQRNN is & Seq. grid is & No statistical \\
  
    & quantiles & speed up &  speed up & saving &  Seq. grid $-$ CQRNN  \\% &  sig. better & sig. better & significant \\
    & & & & & w/ 95\% conf. int. \\
    % & & & & \\% & 95\% conf. interval & in TQMSE? & in TQMSE? & difference \\
    % &&&&& Seq. grid $-$ CQRNN\\
%   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\

\midrule
%   Norm linear &           9 &   14.7$\times$ &   11.2$\times$ &  8.3$\times$ &          -2.189 $\pm$ 0.245 & \checkmark & & \\
 Norm non-linear &           9 &   12.4$\times$ &   9.6$\times$ &  8.3$\times$ &         -0.003 $\pm$ 0.001 \\% & \checkmark & & \\
  Exponential &           9 &   12.4$\times$ &   8.0$\times$ &  8.3$\times$ &           -0.093 $\pm$ 0.176 \\% &  & & \checkmark\\
      Weibull &           9 &   12.5$\times$ &   8.7$\times$ &  8.3$\times$ &         -0.014 $\pm$ 0.016 \\% &  & & \checkmark \\
    %   LogNorm &           9 &   12.9$\times$ &   8.8$\times$ &  8.3$\times$ &         -0.039 $\pm$ 0.028 & \checkmark & & \\
%  Norm uniform$^*$ &           9 &   12.6$\times$ &   8.1$\times$ &  8.3$\times$ &          0.175 $\pm$ 0.033 & & \checkmark  & \\
%   Norm heavy &           19 &  31.0$\times$ &        18.5$\times$ &        16.2$\times$ &           0.108 $\pm$ 0.211 & & & \checkmark\\
    % Norm med. &           19 &  34.1$\times$ &        17.9$\times$ &        16.2$\times$ &          -0.046 $\pm$ 0.004 & \checkmark & & \\
%   Norm light &           19 &  31.7$\times$ &            19.2$\times$ &     16.2$\times$ &         -0.035 $\pm$ 0.003 & \checkmark & & \\
    % Norm same &           19 &  34.3$\times$ &            21.2$\times$ &     16.2$\times$ &         -0.390 $\pm$ 0.049 & \checkmark & & \\
LogNorm heavy &           19 &  33.6$\times$ &        19.9$\times$ &        16.2$\times$ &          0.005 $\pm$ 0.001 \\% & & \checkmark &  \\
%  LogNorm med. &           19 &  31.3$\times$ &        13.1$\times$ &        16.2$\times$ &          0.019 $\pm$ 0.002 & & \checkmark &  \\
LogNorm light &           19 &  31.3$\times$ &        20.2$\times$ &        16.2$\times$ &         -0.033 $\pm$ 0.004 \\% & \checkmark & & \\
%  LogNorm same &           19 &  29.8$\times$ &        18.4$\times$ &        16.2$\times$ &         -0.371 $\pm$ 0.045 & \checkmark & & \\
% \midrule
% \midrule
\bottomrule

\end{tabular}}
\label{tab_grid_cqrnn_compare_mini}
\end{table}

==> QRNN_censored_01(8) copy/tables_figs_etc/table_comparison_real_01.tex <==
\begin{table}[t!]
\centering
\caption{Results comparing CQRNN and sequential grid algorithm on the type 3 datasets, real target data with real censoring. Experiments were repeated over 50 random seeds.}
% To obtain 95\% confidence intervals, we compute the standard error of the difference between means (not assuming independence between samples since random seeds are shared), and multiply it by a two-sided t statistic, with $N-1$ degrees of freedom, at the $\alpha=0.05$ significance level. If zero falls within this confidence interval, the difference is deemed not significant.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}

Raw Results, mean $\pm$ one standard error
\resizebox{0.999\textwidth}{!}{
\begin{tabular}{lllllll}
\toprule
Dataset &          Method & TQMSE & UQL & UnDCal & Concordance-Index (higher better) & Censored D-Calibration (lower better) \\
\midrule
   METABRIC &    CQRNN   &                    - &                  - &      - &         0.643 $\pm$0.003 &         0.218 $\pm$0.026 \\
   METABRIC & Sequential grid &                    - &                  - &      - &         0.648 $\pm$0.002 &          0.399 $\pm$0.04 \\
       WHAS &    CQRNN   &                    - &                  - &      - &          0.86 $\pm$0.002 &         0.721 $\pm$0.091 \\
       WHAS & Sequential grid &                    - &                  - &      - &         0.852 $\pm$0.002 &          5.038 $\pm$0.74 \\
    SUPPORT &    CQRNN   &                    - &                  - &      - &         0.614 $\pm$0.001 &          0.159 $\pm$0.01 \\
    SUPPORT & Sequential grid &                    - &                  - &      - &         0.613 $\pm$0.001 &         0.723 $\pm$0.024 \\
       GBSG &    CQRNN   &                    - &                  - &      - &         0.678 $\pm$0.002 &         0.361 $\pm$0.024 \\
       GBSG & Sequential grid &                    - &                  - &      - &         0.678 $\pm$0.002 &         0.789 $\pm$0.042 \\
  TMBImmuno &    CQRNN   &                    - &                  - &      - &         0.571 $\pm$0.003 &         0.207 $\pm$0.021 \\
  TMBImmuno & Sequential grid &                    - &                  - &      - &         0.572 $\pm$0.003 &         0.375 $\pm$0.028 \\
  BreastMSK &    CQRNN   &                    - &                  - &      - &         0.618 $\pm$0.005 &          0.085 $\pm$0.01 \\
  BreastMSK & Sequential grid &                    - &                  - &      - &         0.597 $\pm$0.006 &         0.227 $\pm$0.016 \\
     LGGGBM &    CQRNN   &                    - &                  - &      - &         0.784 $\pm$0.004 &         0.397 $\pm$0.039 \\
     LGGGBM & Sequential grid &                    - &                  - &      - &         0.781 $\pm$0.004 &         0.491 $\pm$0.041 \\
\bottomrule
\end{tabular}}

\vspace{0.5in}
Difference in means, alongside 95\% confidence interval
\resizebox{0.999\textwidth}{!}{
\begin{tabular}{lrrrrrrrr}
\toprule
Dataset &  Number &  Training time &  Test time &  Parameter & C-Index difference & CQRNN is & CensDCal difference & CQRNN is\\
& quantiles & speed up & speed up & saving & Seq. grid - CQRNN & sig. better? & Seq. grid - CQRNN & sig. better? \\
& & & & & (>0 favours CQRNN) &  & (<0 favours CQRNN) \\
\midrule
%   METABRIC &  5 &    5.3$\times$ &  2.5$\times$ &  0.000 &          -0.0049 $\pm$ 0.0014 &  \\
%       WHAS &  5 &    5.1$\times$ &  3.9$\times$ &  0.000 &           0.0079 $\pm$ 0.0009  & \\
%     SUPPORT &  5 &    5.1$\times$ &  2.7$\times$ &  0.000 &           0.0014 $\pm$ 0.0006  & \\
%       GBSG &  5 &    5.3$\times$ &  5.1$\times$ &  0.000 &          -0.0006 $\pm$ 0.0005 &  \\
%   TMBImmuno &  5 &    5.1$\times$ &  4.3$\times$ &  0.000 &          -0.0006 $\pm$ 0.0013 &  \\
%   BreastMSK &  5 &    5.1$\times$ &  5.0$\times$ &  0.000 &            0.021 $\pm$ 0.0044  & \\
%      LGGGBM &  5 &    5.4$\times$ &  5.1$\times$ &  0.000 &           0.0028 $\pm$ 0.0012  & \\
   METABRIC &  5 & 5.3$\times$ & 2.5$\times$ &  4.6$\times$ & -0.005 $\pm$ 0.001 & \xmark & -0.181 $\pm$ 0.032 & \cmark \\
       WHAS &  5 & 5.1$\times$ & 3.9$\times$ &  4.6$\times$ &  0.008 $\pm$ 0.001  & \cmark & -4.317 $\pm$ 0.745 & \cmark \\
    SUPPORT &  5 & 5.1$\times$ & 2.7$\times$ &  4.6$\times$ &  0.001 $\pm$ 0.000  & \cmark & -0.564 $\pm$ 0.022 & \cmark \\
       GBSG &  5 & 5.3$\times$ & 5.1$\times$ &  4.6$\times$ & -0.001 $\pm$ 0.000 & \xmark & -0.428 $\pm$ 0.026 & \cmark \\
  TMBImmuno &  5 & 5.1$\times$ & 4.3$\times$ &  4.6$\times$ & -0.000 $\pm$ 0.001 & -- & -0.168 $\pm$ 0.025 & \cmark \\
  BreastMSK &  5 & 5.1$\times$ & 5.0$\times$ &  4.6$\times$ &   0.021 $\pm$ 0.004  & \cmark & -0.141 $\pm$ 0.018 & \cmark \\
     LGGGBM &  5 & 5.4$\times$ & 5.1$\times$ &  4.6$\times$ &  0.003 $\pm$ 0.001  & \cmark & -0.094 $\pm$ 0.038 & \cmark \\
\midrule
CQRNN better: & & & & & & 4/7 & & 7/7 \\
Seq grid better: & & & & & & 2/7 & & 0/7 \\
No sig. difference: & & & & & & 1/7 & & 0/7 \\
\bottomrule
\end{tabular}}

% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{lrrrrl}
% \toprule
% dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel & diff\_test\_cens\_Dcal\_cens \\
% \midrule
%   METABRIC &            5 &                   5.271 &                       2.370 &           0.000 &      -0.1814 $\pm$ 0.0319 \\
%       WHAS &            5 &                   5.095 &                       3.911 &           0.000 &      -4.3172 $\pm$ 0.7452 \\
%     SUPPORT &            5 &                   5.112 &                       2.674 &           0.000 &       -0.5635 $\pm$ 0.022 \\
%       GBSG &            5 &                   5.253 &                       5.063 &           0.000 &      -0.4283 $\pm$ 0.0262 \\
%   TMBImmuno &            5 &                   5.130 &                       4.257 &           0.000 &       -0.168 $\pm$ 0.0246 \\
%   BreastMSK &            5 &                   5.089 &                       4.997 &           0.000 &       -0.1414 $\pm$ 0.018 \\
%      LGGGBM &            5 &                   5.394 &                       5.104 &           0.000 &      -0.0939 $\pm$ 0.0377 \\
% \bottomrule
% \end{tabular}}




\label{tab_grid_cqrnn_compare_real}
\end{table}



==> QRNN_censored_01(8) copy/tables_figs_etc/table_dataset_info_02.tex <==
\begin{table}[h!]
\centering
\caption{Summary of all datasets used.}
% See appendix\ref{sec_app_dataset_details} for further detail.
\resizebox{0.9\textwidth}{!}{\begin{tabular}{lrrrrcc}
\toprule
    
     \multicolumn{1}{l}{Dataset} &  \multicolumn{1}{c}{Feats} &  \multicolumn{1}{c}{Train}  &  \multicolumn{1}{c}{Test} &  Prop.  &  Target sampling & Censoring sampling  \\
     
     & & \multicolumn{1}{c}{data} & \multicolumn{1}{c}{data} & censored & distribution  & distribution  \\
\midrule
\multicolumn{7}{c}{\textbf{Type 1 -- Synthetic datasets with synthetic censoring}}\\
     Norm linear &        1 &      500 &    1000 &             0.20 &    $\mathcal{N}(2x+10,(x+1)^2)$ & $\mathcal{N}(4x+10,(0.8x+0.4)^2)$ \\
 Norm non-linear &        1 &      500 &    1000 &             0.24 &    $\mathcal{N}(x\sin(2x)+10,(0.5x+0.5)^2)$ & $\mathcal{N}(2x+10,2^2)$ \\
     Exponential &        1 &      500 &    1000 &             0.30 &    $\operatorname{Exp}(2x+4)$ & $\operatorname{Exp}(-3x+15)$ \\
         Weibull &        1 &      500 &    1000 &             0.22 &    $\operatorname{Weibull}(4x \sin(2(x-1))+10, 5)$ & $\operatorname{Weibull}(-3x+20, 5)$ \\
         LogNorm &        1 &      500 &    1000 &             0.21 &    $\operatorname{Lognorm}((x-1)^2, x^2)$ & $\mathcal{U}(0, 10)$ \\
    Norm uniform &        1 &      500 &    1000 &             0.62 &    $\mathcal{N}(2x \cos(2x)+13,(x^2+0.5)^2)$ & $\mathcal{U}(0, 18)$\\
      Norm heavy &        4 &     2000 &    1000 &             0.80 &   \footnotesize{$\mathcal{N}(3x_0 + x_1^2 - x_2^2 + 2\sin(x_2 x_3)+6,(x^2+0.5)^2)$} & $\mathcal{U}(0, 12)$ \\
      Norm med. &        4 &     2000 &    1000 &             0.49 &    --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 20)$ \\
      Norm light &        4 &     2000 &    1000 &             0.25 &    --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 40)$ \\
      Norm same &        4 &     2000 &    1000 &             0.50 &    --- \raisebox{-0.5ex}{''} --- & Equal to target dist.  \\
  LogNorm heavy &        8 &     4000 &    1000 &             0.75 &    $\operatorname{Lognorm}(\sum_i^8 \beta_i x_i, 1)/10$ & $\mathcal{U}(0, 0.4)$ \\
    LogNorm med. &        8 &     4000 &    1000 &             0.52 &    --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 1.0)$\\
  LogNorm light &        8 &     4000 &    1000 &             0.23 &    --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 3.5)$\\
    LogNorm same &        8 &     4000 &    1000 &             0.50 &    --- \raisebox{-0.5ex}{''} --- & Equal to target dist.  \\
    
        \multicolumn{7}{c}{ \textbf{Type 2 -- Real datasets with synthetic censoring} }\\
         
         Housing &        8 &    16512 &    4128 &             0.50 &    Real & $\mathcal{U}(0, c_1)$ \\
         Protein &        9 &    36584 &    9146 &             0.44 &    Real & $\mathcal{U}(0, c_2)$\\
            Wine &       11 &     5197 &    1300 &             0.69 &    Real & $\mathcal{U}(0, c_3)$\\
             PHM &       21 &    36734 &    9184 &             0.52 &    Real & $\mathcal{U}(0, c_4)$\\
      SurvMNIST &        28$\times$28 &    48000 &   12000 &             0.53  & One Gamma dist. per MNIST class & $\mathcal{U}(0, c_5)$ \\
       
        \multicolumn{7}{c}{ \textbf{Type 3 -- Real datasets with real censoring} }\\
        METABRIC &        9 &     1523 &     381 &             0.42 &    Real & Real \\
            WHAS &        6 &     1310 &     328 &             0.57 &    Real & Real\\
         SUPPORT &       14 &     7098 &    1775 &             0.32 &    Real & Real\\
            GBSG &        7 &     1785 &     447 &             0.42 &    Real & Real\\
      TMBImmuno &        3 &     1328 &     332 &             0.49 &    Real & Real\\
      BreastMSK &        5 &     1467 &     367 &             0.77 &    Real & Real\\
          LGGGBM &        5 &      510 &     128 &             0.60 &    Real & Real\\
\bottomrule
\end{tabular}}
\label{tab_dataset_info}
\end{table}



==> QRNN_censored_01(8) copy/tables_figs_etc/table_dataset_info_02_maxdef.tex <==
\begin{table}[hb]
\centering
\caption{Summary of all datasets used. See appendix \ref{sec_app_dataset_details} for further detail.}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{lrrrrrcc}
\toprule
    
     \multicolumn{1}{l}{Dataset} &  \multicolumn{1}{c}{Feats} &  \multicolumn{1}{c}{Train}  &  \multicolumn{1}{c}{Test} &  Prop.  &  Max defined & Target sampling & Censoring sampling  \\
     
     & & \multicolumn{1}{c}{data} & \multicolumn{1}{c}{data} & censored & global quantile & distribution  & distribution  \\
\midrule
\multicolumn{8}{c}{\textbf{Type 1 -- Synthetic datasets with synthetic censoring}}\\
     Norm linear &        1 &      500 &    1000 &             0.20 &                       0.99 & $\mathcal{N}(2x+10,(x+1)^2)$ & $\mathcal{N}(4x+10,(0.8x+0.4)^2)$ \\
 Norm non-linear &        1 &      500 &    1000 &             0.24 &                       1.00 & $\mathcal{N}(x\sin(2x)+10,(0.5x+0.5)^2)$ & $\mathcal{N}(2x+10,2^2)$ \\
     Exponential &        1 &      500 &    1000 &             0.30 &                       0.99 & $\operatorname{Exp}(2x+4)$ & $\operatorname{Exp}(-3x+15)$ \\
         Weibull &        1 &      500 &    1000 &             0.22 &                       0.97 & $\operatorname{Weibull}(4x \sin(2(x-1))+10, 5)$ & $\operatorname{Weibull}(-3x+20, 5)$ \\
         LogNorm &        1 &      500 &    1000 &             0.21 &                       0.96 & $\operatorname{Lognorm}((x-1)^2, x^2)$ & $\mathcal{U}(0, 10)$ \\
    Norm uniform &        1 &      500 &    1000 &             0.62 &                       0.99 & $\mathcal{N}(2x \cos(2x)+13,(x^2+0.5)^2)$ & $\mathcal{U}(0, 18)$\\
      Norm heavy &        4 &     2000 &    1000 &             0.80 &                       0.75 &  \scriptnotesize $\mathcal{N}(3x_0 + x_1^2 - x_2^2 + 2\sin(x_2 x_3)+6,(x^2+0.5)^2)$ & $\mathcal{U}(0, 12)$ \\
       Norm med. &        4 &     2000 &    1000 &             0.49 &                       1.00 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 20)$ \\
      Norm light &        4 &     2000 &    1000 &             0.25 &                       1.00 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 40)$ \\
       Norm same &        4 &     2000 &    1000 &             0.50 &                       0.98 & --- \raisebox{-0.5ex}{''} --- & Equal to target dist.  \\
   LogNorm heavy &        8 &     4000 &    1000 &             0.75 &                       0.47 & $\operatorname{Lognorm}(\sum_i^8 \beta_i x_i, 1)/10$ & $\mathcal{U}(0, 0.4)$ \\
    LogNorm med. &        8 &     4000 &    1000 &             0.52 &                       0.73 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 1.0)$\\
   LogNorm light &        8 &     4000 &    1000 &             0.23 &                       0.94 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 3.5)$\\
    LogNorm same &        8 &     4000 &    1000 &             0.50 &                       0.99 & --- \raisebox{-0.5ex}{''} --- & Equal to target dist.  \\
    
        \\ \multicolumn{8}{c}{ \textbf{Type 2 -- Real datasets with synthetic censoring} }\\
         
         Housing &        8 &    16512 &    4128 &             0.50 &                       0.90 & Real & $\mathcal{U}(0, c_1)$ \\
         Protein &        9 &    36584 &    9146 &             0.44 &                       0.90 & Real & $\mathcal{U}(0, c_2)$\\
            Wine &       11 &     5197 &    1300 &             0.69 &                       0.90 & Real & $\mathcal{U}(0, c_3)$\\
             PHM &       21 &    36734 &    9184 &             0.52 &                       0.90 & Real & $\mathcal{U}(0, c_4)$\\
       SurvMNIST &        28$\times$28 &    48000 &   12000 &             0.53 &                       0.90 & One Gamma dist. per MNIST class & $\mathcal{U}(0, c_5)$ \\
        
        \\ \multicolumn{8}{c}{ \textbf{Type 3 -- Real datasets with real censoring} }\\
        METABRIC &        9 &     1523 &     381 &             0.42 &                       0.99 & Real & Real \\
            WHAS &        6 &     1310 &     328 &             0.57 &                       0.64 & Real & Real\\
         SUPPORT &       14 &     7098 &    1775 &             0.32 &                       0.76 & Real & Real\\
            GBSG &        7 &     1785 &     447 &             0.42 &                       0.63 & Real & Real\\
       TMBImmuno &        3 &     1328 &     332 &             0.49 &                       0.80 & Real & Real\\
       BreastMSK &        5 &     1467 &     367 &             0.77 &                       0.61 & Real & Real\\
          LGGGBM &        5 &      510 &     128 &             0.60 &                       0.89 & Real & Real\\
\bottomrule
\end{tabular}}
\label{tab_dataset_info}
\end{table}



==> QRNN_censored_01(8) copy/tables_figs_etc/table_main_results_03.tex <==
\begin{table}[ht]
\centering
\caption{Full results table for all datasets, methods and metrics. Mean $\pm$ 1 standard error for test set over 10 runs.} 
\resizebox{1.\textwidth}{!}{\begin{tabular}{lllllll}
\toprule
     Dataset &        Method & MSE to true quantile & Uncensored quantile loss & Uncensored D-Calibration & Concordance-Index & Censored D-Calibration  \\
     
      &     &  (lower better) & (lower better) & (lower better) & (higher better) & (lower better)  \\


\midrule
&\multicolumn{6}{c}{\textbf{Type 1 -- synthetic data, synthetic censoring}}\\

   Norm linear &            CQRNN &                      \textbf{0.088 $\pm$ 0.009} &                            \textbf{1.517 $\pm$0.01} &          0.327 $\pm$0.057 &                     \textbf{0.663 $\pm$0.002} &                         \textbf{0.211 $\pm$0.034} \\
   Norm linear &  Sequential grid &                      2.779 $\pm$ 0.506 &                            1.623 $\pm$0.02 &           \textbf{0.303 $\pm$0.06} &                     0.662 $\pm$0.002 &                         0.224 $\pm$0.024 \\
   Norm linear &     Excl. censor &                      0.566 $\pm$ 0.039 &                            1.62 $\pm$0.016 &          3.078 $\pm$0.244 &                     0.662 $\pm$0.002 &                         2.349 $\pm$0.102 \\
   Norm linear &     DeepQuantReg &                      1.172 $\pm$ 0.133 &                           1.695 $\pm$0.026 &           1.94 $\pm$0.192 &                     \textbf{0.663 $\pm$0.002} &                         1.241 $\pm$0.138 \\
   Norm linear &      LogNorm MLE &                      0.184 $\pm$ 0.021 &                           1.522 $\pm$0.008 &          0.315 $\pm$0.023 &                     0.662 $\pm$0.002 &                          0.232 $\pm$0.04 \\
   
   \midrule
   
  Norm non-lin &            CQRNN &                      0.028 $\pm$ 0.004 &                           \textbf{0.759 $\pm$0.005} &          \textbf{0.262 $\pm$0.044} &                     \textbf{0.674 $\pm$0.004} &                         \textbf{0.186 $\pm$0.023} \\
  Norm non-lin &  Sequential grid &                      \textbf{0.027 $\pm$ 0.003} &                           \textbf{0.759 $\pm$0.005} &          0.283 $\pm$0.034 &                     0.673 $\pm$0.004 &                          0.194 $\pm$0.03 \\
  Norm non-lin &     Excl. censor &                      0.053 $\pm$ 0.004 &                           0.768 $\pm$0.006 &          0.579 $\pm$0.088 &                     0.673 $\pm$0.004 &                         0.449 $\pm$0.054 \\
  Norm non-lin &     DeepQuantReg &                      0.818 $\pm$ 0.093 &                           0.998 $\pm$0.019 &          4.263 $\pm$0.234 &                     0.609 $\pm$0.023 &                         2.593 $\pm$0.206 \\
  Norm non-lin &      LogNorm MLE &                      0.323 $\pm$ 0.035 &                           0.824 $\pm$0.009 &          1.651 $\pm$0.118 &                     0.653 $\pm$0.005 &                         0.971 $\pm$0.077 \\
  
  \midrule
  
   Exponential &            CQRNN &                      \textbf{1.298 $\pm$ 0.201} &                            \textbf{4.057 $\pm$0.04} &          0.404 $\pm$0.035 &                     \textbf{0.559 $\pm$0.003} &                         0.248 $\pm$0.031 \\
   Exponential &  Sequential grid &                      1.702 $\pm$ 0.397 &                           4.061 $\pm$0.039 &          \textbf{0.391 $\pm$0.057} &                     0.558 $\pm$0.004 &                         \textbf{0.226 $\pm$0.025} \\
   Exponential &     Excl. censor &                      11.03 $\pm$ 0.772 &                           4.456 $\pm$0.039 &           2.537 $\pm$0.18 &                     0.535 $\pm$0.007 &                          1.513 $\pm$0.14 \\
   Exponential &     DeepQuantReg &                     20.046 $\pm$ 5.844 &                            4.675 $\pm$0.09 &          2.294 $\pm$0.252 &                     0.544 $\pm$0.004 &                         1.276 $\pm$0.158 \\
   Exponential &      LogNorm MLE &                     17.825 $\pm$ 2.831 &                           4.342 $\pm$0.058 &          1.056 $\pm$0.071 &                     0.552 $\pm$0.003 &                         0.401 $\pm$0.045 \\
     
  \midrule
  
       Weibull &            CQRNN &                      \textbf{0.255 $\pm$ 0.025} &                           1.879 $\pm$0.018 &           \textbf{0.33 $\pm$0.037} &                     \textbf{0.772 $\pm$0.002} &                         0.211 $\pm$0.023 \\
       Weibull &  Sequential grid &                      0.261 $\pm$ 0.018 &                           \textbf{1.877 $\pm$0.017} &          0.352 $\pm$0.037 &                     \textbf{0.772 $\pm$0.002} &                         \textbf{0.209 $\pm$0.023} \\
       Weibull &     Excl. censor &                      2.468 $\pm$ 0.118 &                            2.18 $\pm$0.021 &          1.942 $\pm$0.152 &                     0.769 $\pm$0.002 &                         0.834 $\pm$0.069 \\
       Weibull &     DeepQuantReg &                       1.116 $\pm$ 0.16 &                           2.005 $\pm$0.037 &          1.057 $\pm$0.159 &                     0.769 $\pm$0.002 &                         0.556 $\pm$0.126 \\
       Weibull &      LogNorm MLE &                      1.586 $\pm$ 0.081 &                            2.048 $\pm$0.02 &          0.603 $\pm$0.036 &                     0.771 $\pm$0.002 &                         0.478 $\pm$0.072 \\
         
  \midrule
  
       LogNorm &            CQRNN &                      0.411 $\pm$ 0.057 &                            1.716 $\pm$0.04 &          0.253 $\pm$0.025 &                      0.59 $\pm$0.004 &                         0.161 $\pm$0.015 \\
       LogNorm &  Sequential grid &                      0.328 $\pm$ 0.036 &                           1.716 $\pm$0.041 &           0.28 $\pm$0.033 &                     \textbf{0.591 $\pm$0.003} &                         0.193 $\pm$0.024 \\
       LogNorm &     Excl. censor &                      1.757 $\pm$ 0.114 &                           1.818 $\pm$0.051 &           1.46 $\pm$0.129 &                     0.588 $\pm$0.004 &                         1.119 $\pm$0.062 \\
       LogNorm &     DeepQuantReg &                      1.279 $\pm$ 0.168 &                            1.843 $\pm$0.04 &          1.924 $\pm$0.131 &                      0.58 $\pm$0.004 &                         1.279 $\pm$0.106 \\
       LogNorm &      LogNorm MLE &                      \textbf{0.247 $\pm$ 0.032} &                           \textbf{1.713 $\pm$0.041} &          \textbf{0.115 $\pm$0.014} &                     0.589 $\pm$0.004 &                         \textbf{0.151 $\pm$0.018} \\
         
  \midrule
  
  Norm uniform &            CQRNN &                      0.388 $\pm$ 0.054 &                           1.442 $\pm$0.022 &          2.219 $\pm$0.212 &                     0.789 $\pm$0.003 &                        \textbf{0.094 $\pm$0.008} \\
  Norm uniform &  Sequential grid &                     \textbf{ 0.188 $\pm$ 0.016} &                          \textbf{ 1.409 $\pm$0.017} &         \textbf{ 1.347 $\pm$0.136} &                     0.788 $\pm$0.003 &                          0.462 $\pm$0.02 \\
  Norm uniform &     Excl. censor &                      1.088 $\pm$ 0.112 &                           1.501 $\pm$0.018 &           1.557 $\pm$0.19 &                      \textbf{0.79 $\pm$0.003} &                         0.721 $\pm$0.066 \\
  Norm uniform &     DeepQuantReg &                       2.591 $\pm$ 0.56 &                           1.809 $\pm$0.084 &          4.397 $\pm$0.687 &                     0.598 $\pm$0.064 &                         0.418 $\pm$0.074 \\
  Norm uniform &      LogNorm MLE &                   939.992 $\pm$ 144.76 &                           7.727 $\pm$0.502 &         32.486 $\pm$1.405 &                      0.77 $\pm$0.006 &                         4.259 $\pm$0.144 \\
    
  \midrule
  
    Norm heavy &            CQRNN &                      \textbf{0.579 $\pm$ 0.089} &                           0.999 $\pm$0.041 &          \textbf{6.491 $\pm$1.094} &                     0.922 $\pm$0.002 &                         0.301 $\pm$0.067 \\
    Norm heavy &  Sequential grid &                      0.597 $\pm$ 0.081 &                           \textbf{0.996 $\pm$0.037} &          6.595 $\pm$1.406 &                     \textbf{0.923 $\pm$0.002} &                         {0.198 $\pm$0.014} \\
    Norm heavy &     Excl. censor &                      1.285 $\pm$ 0.205 &                           1.223 $\pm$0.069 &          8.206 $\pm$1.895 &                     \textbf{0.923 $\pm$0.002} &                         0.261 $\pm$0.021 \\
    Norm heavy &     DeepQuantReg &                      1.099 $\pm$ 0.175 &                            1.166 $\pm$0.06 &          6.681 $\pm$1.365 &                     \textbf{0.923 $\pm$0.002} &                         \textbf{0.191 $\pm$0.016} \\
    Norm heavy &      LogNorm MLE &                5568.886 $\pm$ 1737.861 &                          17.077 $\pm$2.442 &         21.283 $\pm$1.057 &                     0.852 $\pm$0.008 &                         1.113 $\pm$0.102 \\
      
  \midrule
  
     Norm med. &            CQRNN &                       \textbf{0.11 $\pm$ 0.007} &                           \textbf{0.789 $\pm$0.006} &          0.633 $\pm$0.138 &                     \textbf{0.896 $\pm$0.001} &                         {0.157 $\pm$0.054} \\
     Norm med. &  Sequential grid &                       0.16 $\pm$ 0.009 &                           0.799 $\pm$0.005 &          0.474 $\pm$0.046 &                     0.895 $\pm$0.001 &                         0.159 $\pm$0.011 \\
     Norm med. &     Excl. censor &                      0.117 $\pm$ 0.008 &                           0.792 $\pm$0.005 &           \textbf{0.247 $\pm$0.02} &                     \textbf{0.896 $\pm$0.001} &                        \textbf{0.136 $\pm$0.015} \\
     Norm med. &     DeepQuantReg &                      0.255 $\pm$ 0.016 &                           0.847 $\pm$0.008 &          0.944 $\pm$0.098 &                     0.892 $\pm$0.001 &                         0.232 $\pm$0.029 \\
     Norm med. &      LogNorm MLE &                   276.276 $\pm$ 41.622 &                           3.974 $\pm$0.228 &         17.969 $\pm$0.548 &                     0.865 $\pm$0.004 &                         4.612 $\pm$0.134 \\
       
  \midrule
  
    Norm light &            CQRNN &                      \textbf{0.079 $\pm$ 0.005} &                           \textbf{0.778 $\pm$0.005} &          0.173 $\pm$0.021 &                     \textbf{0.882 $\pm$0.001} &                         \textbf{0.084 $\pm$0.008} \\
    Norm light &  Sequential grid &                      0.117 $\pm$ 0.005 &                           0.784 $\pm$0.004 &          0.352 $\pm$0.027 &                     \textbf{0.882 $\pm$0.001} &                          0.19 $\pm$0.018 \\
    Norm light &     Excl. censor &                      0.083 $\pm$ 0.005 &                           0.779 $\pm$0.005 &          \textbf{0.159 $\pm$0.017} &                    \textbf{0.882 $\pm$0.001} &                         0.112 $\pm$0.013 \\
    Norm light &     DeepQuantReg &                      0.277 $\pm$ 0.013 &                           0.854 $\pm$0.008 &          1.205 $\pm$0.081 &                     0.878 $\pm$0.001 &                         0.588 $\pm$0.046 \\
    Norm light &      LogNorm MLE &                     58.503 $\pm$ 6.922 &                           2.475 $\pm$0.093 &         13.713 $\pm$0.465 &                     0.861 $\pm$0.003 &                          7.74 $\pm$0.286 \\
      
  \midrule
  
     Norm same &            CQRNN &                      \textbf{0.094 $\pm$ 0.005} &                           \textbf{0.785 $\pm$0.003} &           0.19 $\pm$0.022 &                     0.893 $\pm$0.001 &                         \textbf{0.052 $\pm$0.007} \\
     Norm same &  Sequential grid &                       0.779 $\pm$ 0.16 &                           0.847 $\pm$0.009 &           0.45 $\pm$0.054 &                     0.891 $\pm$0.001 &                         0.102 $\pm$0.012 \\
     Norm same &     Excl. censor &                       0.435 $\pm$ 0.01 &                           0.927 $\pm$0.007 &          4.096 $\pm$0.251 &                     \textbf{0.894 $\pm$0.001} &                          1.398 $\pm$0.07 \\
     Norm same &     DeepQuantReg &                      0.357 $\pm$ 0.013 &                           0.893 $\pm$0.009 &          3.334 $\pm$0.325 &                     0.891 $\pm$0.001 &                         0.983 $\pm$0.091 \\
     Norm same &      LogNorm MLE &                      0.114 $\pm$ 0.008 &                           0.787 $\pm$0.004 &         \textbf{ 0.187 $\pm$0.024} &                     \textbf{0.894 $\pm$0.001} &                         0.059 $\pm$0.006 \\
            
  \midrule
  
 LogNorm heavy &            CQRNN &                      2.424 $\pm$ 0.055 &                           1.123 $\pm$0.021 &          22.493 $\pm$0.36 &                     \textbf{0.782 $\pm$0.005} &                         \textbf{0.036 $\pm$0.004} \\
 LogNorm heavy &  Sequential grid &                       2.42 $\pm$ 0.055 &                           1.121 $\pm$0.021 &         21.938 $\pm$0.299 &                     0.781 $\pm$0.005 &                         0.044 $\pm$0.002 \\
 LogNorm heavy &     Excl. censor &                      2.654 $\pm$ 0.061 &                           1.247 $\pm$0.021 &          35.43 $\pm$0.629 &                     0.772 $\pm$0.005 &                         4.806 $\pm$0.226 \\
 LogNorm heavy &     DeepQuantReg &                       2.639 $\pm$ 0.06 &                           1.236 $\pm$0.022 &         34.132 $\pm$0.719 &                     0.771 $\pm$0.005 &                         3.884 $\pm$0.201 \\
 LogNorm heavy &      LogNorm MLE &                       \textbf{1.17 $\pm$ 0.052} &                           \textbf{0.868 $\pm$0.018} &          \textbf{0.135 $\pm$0.014} &                     0.766 $\pm$0.005 &                         0.074 $\pm$0.008 \\
        
  \midrule
  
  LogNorm med. &            CQRNN &                      1.713 $\pm$ 0.049 &                            0.923 $\pm$0.02 &          5.054 $\pm$0.174 &                     \textbf{0.754 $\pm$0.004} &                         \textbf{0.064 $\pm$0.005} \\
  LogNorm med. &  Sequential grid &                      1.699 $\pm$ 0.047 &                            0.921 $\pm$0.02 &          4.968 $\pm$0.181 &                     \textbf{0.754 $\pm$0.004} &                         0.098 $\pm$0.014 \\
  LogNorm med. &     Excl. censor &                      2.168 $\pm$ 0.053 &                           1.067 $\pm$0.021 &          12.124 $\pm$0.34 &                     0.749 $\pm$0.004 &                         2.586 $\pm$0.071 \\
  LogNorm med. &     DeepQuantReg &                      2.087 $\pm$ 0.056 &                            1.033 $\pm$0.02 &         10.081 $\pm$0.255 &                     0.748 $\pm$0.003 &                         1.373 $\pm$0.055 \\
  LogNorm med. &      LogNorm MLE &                       \textbf{0.907 $\pm$ 0.05} &                           \textbf{0.824 $\pm$0.018} &          \textbf{0.103 $\pm$0.016} &                      0.75 $\pm$0.003 &                          0.07 $\pm$0.009 \\
         
  \midrule
  
 LogNorm light &            CQRNN &                      0.506 $\pm$ 0.028 &                           \textbf{0.764 $\pm$0.019} &          0.331 $\pm$0.026 &                     \textbf{0.729 $\pm$0.003} &                          0.135 $\pm$0.01 \\
 LogNorm light &  Sequential grid &                      0.532 $\pm$ 0.029 &                           0.767 $\pm$0.018 &           0.517 $\pm$0.04 &                     \textbf{0.729 $\pm$0.003} &                          0.21 $\pm$0.014 \\
 LogNorm light &     Excl. censor &                      1.185 $\pm$ 0.037 &                            0.852 $\pm$0.02 &          1.518 $\pm$0.124 &                     \textbf{0.729 $\pm$0.003} &                         0.655 $\pm$0.047 \\
 LogNorm light &     DeepQuantReg &                      0.831 $\pm$ 0.036 &                           0.804 $\pm$0.019 &          0.912 $\pm$0.061 &                     0.726 $\pm$0.003 &                         0.438 $\pm$0.028 \\
 LogNorm light &      LogNorm MLE &                      \textbf{0.432 $\pm$ 0.034} &                           0.767 $\pm$0.018 &          \textbf{0.095 $\pm$0.015} &                     \textbf{0.729 $\pm$0.002} &                         \textbf{0.079 $\pm$0.004} \\
        
  \midrule
  
  LogNorm same &            CQRNN &                      0.137 $\pm$ 0.021 &                           0.735 $\pm$0.015 &          0.236 $\pm$0.021 &                     0.751 $\pm$0.002 &                         0.055 $\pm$0.007 \\
  LogNorm same &  Sequential grid &                      0.422 $\pm$ 0.054 &                           0.753 $\pm$0.016 &          0.463 $\pm$0.046 &                     0.752 $\pm$0.003 &                         0.101 $\pm$0.018 \\
  LogNorm same &     Excl. censor &                      1.068 $\pm$ 0.043 &                           0.861 $\pm$0.019 &          4.112 $\pm$0.264 &                     0.752 $\pm$0.002 &                         1.306 $\pm$0.046 \\
  LogNorm same &     DeepQuantReg &                      0.394 $\pm$ 0.057 &                           0.763 $\pm$0.016 &          1.301 $\pm$0.265 &                     0.748 $\pm$0.002 &                         0.335 $\pm$0.072 \\
  LogNorm same &      LogNorm MLE &                      \textbf{0.067 $\pm$ 0.013} &                            \textbf{0.73 $\pm$0.015} &         \textbf{ 0.114 $\pm$0.013} &                     \textbf{0.754 $\pm$0.002} &                         \textbf{0.052 $\pm$0.005} \\
         
  \midrule
  
  
  
  
\end{tabular}}
\label{tab_full_resultsa}
% \caption{Full results table for all datasets, methods and metrics. Mean $\pm$ 1 standard error over 10 runs.} 
\end{table} 

  \newpage
  
  \begin{table}[ht]
\centering
\resizebox{1.\textwidth}{!}{\begin{tabular}{lllllll}
\toprule
     Dataset &        Method & MSE to true quantile & Uncensored quantile loss & Uncensored D-Calibration & Concordance-Index & Censored D-Calibration  \\
     
      &     &  (lower better) & (lower better) & (lower better) & (higher better) & (lower better)  \\


\midrule
&\multicolumn{6}{c}{\textbf{Type 2 -- real data, synthetic censoring}}\\
       Housing &            CQRNN &                                     - &                            \textbf{0.34 $\pm$0.002} &           \textbf{0.793 $\pm$0.03} &                       0.897 $\pm$0.0 &                          \textbf{0.02 $\pm$0.004} \\
       Housing &     Excl. censor &                                     - &                           0.443 $\pm$0.005 &          2.176 $\pm$0.057 &                     0.895 $\pm$0.001 &                         0.311 $\pm$0.011 \\
       Housing &     DeepQuantReg &                                     - &                           0.399 $\pm$0.004 &          2.474 $\pm$0.066 &                     \textbf{0.902 $\pm$0.001} &                         0.196 $\pm$0.031 \\
       Housing &      LogNorm MLE &                                     - &                             0.6 $\pm$0.002 &          2.794 $\pm$0.022 &                     0.881 $\pm$0.001 &                         1.035 $\pm$0.015 \\
       
       \midrule
       
       Protein &            CQRNN &                                     - &                           \textbf{0.435 $\pm$0.001} &          \textbf{0.275 $\pm$0.008} &                     \textbf{0.847 $\pm$0.001} &                         \textbf{0.027 $\pm$0.001} \\
       Protein &     Excl. censor &                                     - &                           0.631 $\pm$0.002 &           3.45 $\pm$0.053 &                     0.838 $\pm$0.001 &                          1.075 $\pm$0.02 \\
       Protein &     DeepQuantReg &                                     - &                           0.568 $\pm$0.002 &          2.809 $\pm$0.059 &                     0.831 $\pm$0.001 &                         0.495 $\pm$0.011 \\
       Protein &      LogNorm MLE &                                     - &                           0.579 $\pm$0.002 &          0.694 $\pm$0.018 &                     0.817 $\pm$0.002 &                         0.298 $\pm$0.007 \\
              
       \midrule
       
          Wine &            CQRNN &                                     - &                             \textbf{0.6 $\pm$0.005} &          \textbf{0.908 $\pm$0.069} &                     \textbf{0.815 $\pm$0.002} &                         \textbf{0.046 $\pm$0.005} \\
          Wine &     Excl. censor &                                     - &                           0.791 $\pm$0.005 &          6.606 $\pm$0.209 &                     0.799 $\pm$0.003 &                         0.722 $\pm$0.038 \\
          Wine &     DeepQuantReg &                                     - &                           0.717 $\pm$0.005 &          3.211 $\pm$0.159 &                     0.792 $\pm$0.003 &                         0.212 $\pm$0.021 \\
          Wine &      LogNorm MLE &                                     - &                           1.454 $\pm$0.022 &          5.736 $\pm$0.163 &                     0.747 $\pm$0.004 &                         0.784 $\pm$0.022 \\
                 
       \midrule
       
           PHM &            CQRNN &                                     - &                           \textbf{0.408 $\pm$0.001} &          \textbf{0.243 $\pm$0.012} &                     \textbf{0.902 $\pm$0.001} &                         \textbf{0.008 $\pm$0.001} \\
           PHM &     Excl. censor &                                     - &                           0.519 $\pm$0.002 &          3.852 $\pm$0.037 &                     0.901 $\pm$0.001 &                         0.481 $\pm$0.006 \\
           PHM &     DeepQuantReg &                                     - &                           0.479 $\pm$0.002 &          1.589 $\pm$0.057 &                     0.897 $\pm$0.001 &                         0.154 $\pm$0.011 \\
           PHM &      LogNorm MLE &                                     - &                           0.599 $\pm$0.002 &           2.26 $\pm$0.018 &                       0.9 $\pm$0.001 &                         0.538 $\pm$0.007 \\
                  
       \midrule
       
     SurvMNIST &            CQRNN &                                     - &                             \textbf{0.076 $\pm$0.0} &          \textbf{0.308 $\pm$0.023} &                     0.899 $\pm$0.001 &                         \textbf{0.224 $\pm$0.005} \\
     SurvMNIST &     Excl. censor &                                     - &                           0.133 $\pm$0.002 &          2.115 $\pm$0.086 &                     0.896 $\pm$0.001 &                         0.512 $\pm$0.014 \\
     SurvMNIST &     DeepQuantReg &                                     - &                             0.1 $\pm$0.001 &          1.021 $\pm$0.051 &                       \textbf{0.9 $\pm$0.001} &                         0.264 $\pm$0.013 \\
     SurvMNIST &      LogNorm MLE &                                     - &                           0.209 $\pm$0.001 &          4.348 $\pm$0.049 &                     0.894 $\pm$0.001 &                         0.806 $\pm$0.015 \\
            
       \midrule \\
       &\multicolumn{6}{c}{\textbf{Type 3 -- real data, real censoring}}\\
      METABRIC &            CQRNN &                                     - &                                         - &                        - &                     \textbf{0.644 $\pm$0.006} &                         \textbf{0.189 $\pm$0.057} \\
      METABRIC &     Excl. censor &                                     - &                                         - &                        - &                     0.615 $\pm$0.005 &                          7.54 $\pm$0.478 \\
      METABRIC &     DeepQuantReg &                                     - &                                         - &                        - &                     0.601 $\pm$0.006 &                         2.393 $\pm$0.211 \\
      METABRIC &      LogNorm MLE &                                     - &                                         - &                        - &                     0.636 $\pm$0.006 &                          0.72 $\pm$0.106 \\
             
       \midrule
       
          WHAS &            CQRNN &                                     - &                                         - &                        - &                      \textbf{0.85 $\pm$0.005} &                         1.089 $\pm$0.431 \\
          WHAS &     Excl. censor &                                     - &                                         - &                        - &                     0.785 $\pm$0.006 &                         9.391 $\pm$0.709 \\
          WHAS &     DeepQuantReg &                                     - &                                         - &                        - &                     0.774 $\pm$0.008 &                          6.71 $\pm$0.448 \\
          WHAS &      LogNorm MLE &                                     - &                                         - &                        - &                      0.81 $\pm$0.005 &                         \textbf{0.817 $\pm$0.139} \\
                 
       \midrule
       
       SUPPORT &            CQRNN &                                     - &                                         - &                        - &                     0.615 $\pm$0.002 &                         \textbf{0.179 $\pm$0.022} \\
       SUPPORT &     Excl. censor &                                     - &                                         - &                        - &                     0.552 $\pm$0.002 &                         9.606 $\pm$0.231 \\
       SUPPORT &     DeepQuantReg &                                     - &                                         - &                        - &                     0.564 $\pm$0.002 &                         6.747 $\pm$0.176 \\
       SUPPORT &      LogNorm MLE &                                     - &                                         - &                        - &                     \textbf{0.617 $\pm$0.002} &                         2.384 $\pm$0.143 \\
              
       \midrule
       
          GBSG &            CQRNN &                                     - &                                         - &                        - &                     \textbf{0.683 $\pm$0.005} &                         \textbf{0.339 $\pm$0.033} \\
          GBSG &     Excl. censor &                                     - &                                         - &                        - &                     0.673 $\pm$0.005 &                        11.732 $\pm$0.512 \\
          GBSG &     DeepQuantReg &                                     - &                                         - &                        - &                     0.673 $\pm$0.005 &                         8.998 $\pm$0.479 \\
          GBSG &      LogNorm MLE &                                     - &                                         - &                        - &                     0.677 $\pm$0.004 &                          0.793 $\pm$0.08 \\
                 
       \midrule
       
     TMBImmuno &            CQRNN &                                     - &                                         - &                        - &                     0.579 $\pm$0.008 &                          \textbf{0.201 $\pm$0.04} \\
     TMBImmuno &     Excl. censor &                                     - &                                         - &                        - &                      0.52 $\pm$0.008 &                         9.479 $\pm$0.386 \\
     TMBImmuno &     DeepQuantReg &                                     - &                                         - &                        - &                     0.539 $\pm$0.011 &                         4.827 $\pm$0.306 \\
     TMBImmuno &      LogNorm MLE &                                     - &                                         - &                        - &                     \textbf{0.581 $\pm$0.007} &                         0.634 $\pm$0.067 \\
            
       \midrule
       
     BreastMSK &            CQRNN &                                     - &                                         - &                        - &                      0.619 $\pm$0.01 &                          \textbf{0.08 $\pm$0.012} \\
     BreastMSK &     Excl. censor &                                     - &                                         - &                        - &                     \textbf{0.646 $\pm$0.008} &                         4.546 $\pm$0.235 \\
     BreastMSK &     DeepQuantReg &                                     - &                                         - &                        - &                     0.638 $\pm$0.008 &                            3.0 $\pm$0.17 \\
     BreastMSK &      LogNorm MLE &                                     - &                                         - &                        - &                      0.631 $\pm$0.01 &                         0.521 $\pm$0.058 \\
            
       \midrule
       
        LGGGBM &            CQRNN &                                     - &                                         - &                        - &                     0.792 $\pm$0.008 &                         0.372 $\pm$0.074 \\
        LGGGBM &     Excl. censor &                                     - &                                         - &                        - &                      0.782 $\pm$0.01 &                         2.166 $\pm$0.303 \\
        LGGGBM &     DeepQuantReg &                                     - &                                         - &                        - &                     0.781 $\pm$0.011 &                         1.275 $\pm$0.184 \\
        LGGGBM &      LogNorm MLE &                                     - &                                         - &                        - &                     \textbf{0.793 $\pm$0.008} &                         \textbf{0.367 $\pm$0.083} \\
\bottomrule



\end{tabular}}
\label{tab_full_results}

\end{table} 

==> QRNN_censored_01(8) copy/tables_figs_etc/table_ymax_01.tex <==
\begin{table}[ht]
\centering
\caption{Ablation over psuedo y value, $y^*$. Mean over ten runs, all hyperparameters fixed. } 
\resizebox{0.7\textwidth}{!}{\begin{tabular}{lrrrrrr}
\toprule
    &  \multicolumn{6}{c}{----- Target value for pseudo-datapoints, $y^*$ -----}\\
   Dataset & \small $1.0\max_i y_i$ &  \small  $1.2 \max_i y_i$ &  \small  $1.5 \max_i y_i$ &  \small  $2.0 \max_i y_i$ &  \small   $10.0 \max_i y_i$ &  \small    $100.0 \max_i y_i$ \\
\midrule
 
& \multicolumn{6}{c}{\textbf{TQMSE (lower better)}}\\

    Norm heavy & 1.452 & 0.579 & 1.237 & 6.196 & 591.257 & 57421.824 \\
    Norm light & 0.081 & 0.079 & 0.081 & 0.081 &   0.081 &     0.081 \\
 LogNorm heavy & 2.502 & 2.424 & 2.321 & 2.173 &   1.026 &    19.827 \\
 LogNorm light & 0.614 & 0.506 & 0.385 & 0.252 &   0.147 &     0.147 \\


% \\
% & \multicolumn{6}{c}{\textbf{Uncensored quantile loss 
% (lower better)}}\\

%     Norm heavy & 1.314 & 0.999 & 1.243 & 2.272 & 16.950 & 149.074 \\
%     Norm light & 0.778 & 0.778 & 0.778 & 0.778 &  0.778 &   0.778 \\
%  LogNorm heavy & 1.152 & 1.123 & 1.088 & 1.045 &  0.860 &   2.432 \\
%  LogNorm light & 0.772 & 0.764 & 0.756 & 0.748 &  0.741 &   0.741 \\



% \\
% & \multicolumn{6}{c}{\textbf{Uncensored D-Calibration (lower better)}} \\

%     Norm heavy &  9.852 &  6.491 &  9.671 & 13.564 & 17.001 & 21.640 \\
%     Norm light &  0.185 &  0.173 &  0.188 &  0.187 &  0.189 &  0.189 \\
%  LogNorm heavy & 26.081 & 22.493 & 18.465 & 15.182 &  4.244 &  5.103 \\
%  LogNorm light &  0.405 &  0.331 &  0.281 &  0.226 &  0.188 &  0.188 \\


% \\
% & \multicolumn{6}{c}{\textbf{Concordance-Index 
% (higher better)}}\\

%     Norm heavy & 0.920 & 0.922 & 0.922 & 0.921 & 0.918 &  0.917 \\
%     Norm light & 0.882 & 0.882 & 0.882 & 0.882 & 0.882 &  0.882 \\
%  LogNorm heavy & 0.780 & 0.782 & 0.784 & 0.784 & 0.783 &  0.782 \\
%  LogNorm light & 0.729 & 0.729 & 0.729 & 0.729 & 0.729 &  0.729 \\


% \\
% & \multicolumn{6}{c}{\textbf{Censored D-Calibration 
% (lower better)}}\\

%     Norm heavy & 0.238 & 0.301 & 0.150 & 0.112 & 0.121 &  0.054 \\
%     Norm light & 0.086 & 0.084 & 0.091 & 0.089 & 0.086 &  0.086 \\
%  LogNorm heavy & 0.094 & 0.036 & 0.033 & 0.030 & 0.028 &  0.099 \\
%  LogNorm light & 0.119 & 0.135 & 0.119 & 0.136 & 0.122 &  0.122 \\

\bottomrule
\end{tabular}}
\label{tab_ymax}
\end{table} 


==> tables_figs_etc/fig_1D_02.tex <==
\begin{figure}[h!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

\small CQRNN (ours) \hspace{0.6in}  Excl. censor \hspace{0.6in}  DeepQuantReg \hspace{0.6in}  LogNorm MLE


\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_cqrnn_v01.pdf}
\put(-107,2){\rotatebox{90}{\small Norm1D uniform}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_uniform_lognorm_v01.pdf}
\put(-0,4){\transparent{1.}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}
% \put(-42,4){\transparent{0.9}\includegraphics[width=0.1\columnwidth]{images/1D_plots/1Dinput_legend_01.pdf}}


\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_cqrnn_v01.pdf}
\put(-107,7){\rotatebox{90}{\small Norm1D linear}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_lognorm_v01.pdf}

\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_cqrnn_v01.pdf}
\put(-107,5){\rotatebox{90}{\small Norm1D non-lin.}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Gaussian_linear_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Gaussian_nonlinear_lognorm_v01.pdf}


\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_cqrnn_v01.pdf}
\put(-107,8){\rotatebox{90}{\small Exponential1D}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Exponential_lognorm_v01.pdf}

\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_cqrnn_v01.pdf}
\put(-107,18){\rotatebox{90}{\small Weibull1D}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_Weibull_lognorm_v01.pdf}

\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_cqrnn_v01.pdf}
\put(-107,10){\rotatebox{90}{\small LogNorm1D}}
% \includegraphics[width=0.19\columnwidth]{images/1D_plots/1Dinput_Exponential_neocleous_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_excl_censor_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_deepquantreg_v01.pdf}
\includegraphics[width=0.245\columnwidth]{images/1D_plots/1Dinput_LogNorm_lognorm_v01.pdf}





\caption{This figure shows estimated quantiles (blue through pink) compared to ground truth quantiles (dashed black lines).
It shows 1D synthetic datasets of varying functions and noise distributions (rows), fitted by various methods (columns).
% described in table \ref{tab_dataset_info}
CQRNN recovers quantiles closest to the ground truth on most datasets.}
\label{fig_1D_plots}
\end{center}
\vskip -0.2in
\end{figure}

==> tables_figs_etc/fig_bench_cindex_dcal_02.tex <==
\begin{figure}[t!]
%\vskip -0.1in
\begin{center}
%a) Low-dimensional input, shallow network \hspace{0.5in} b) High-dimensional input, deep network 
\vspace{-0.02in}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_legend_synth_1D_test_q_metric_selected_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_ND_test_q_metric_selected_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_cens_test_quantile_sum_v01.pdf}

% \includegraphics[width=0.7\columnwidth]{images/main_results/mainresults_synth_cens_test_Dcal_nocens_v01.pdf}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_1D_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_1D_test_cens_Dcal_cens_v01.pdf}
\put(-0,15){\transparent{1.}\includegraphics[width=0.1\columnwidth]{images/main_results/mainresults_legend_01.pdf}}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_ND_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_ND_test_cens_Dcal_cens_v01.pdf}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_cens_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_synth_cens_test_cens_Dcal_cens_v01.pdf}

\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_real_cens_test_cens_cindex_median_v01.pdf}
\includegraphics[width=0.49\columnwidth]{images/main_results/mainresults_real_cens_test_cens_Dcal_cens_v01.pdf}

\caption{Main results. Mean $\pm$ one standard error over ten runs. See table \ref{tab_full_results} for further assessed metrics.}
\label{fig_metric_plots_cindex_dcal}
\end{center}
\vskip -0.2in
\end{figure}

==> tables_figs_etc/table_comparison_grid_01.tex <==
\begin{table}[ht]
\centering
\resizebox{1.\textwidth}{!}{\begin{tabular}{lrrrrrrr}

\toprule
%   dataset\_str &  diff\_time\_training\_time &  diff\_time\_test\_fwdpass\_time &  diff\_test\_q\_metric\_selected &  diff\_test\_quantile\_sum &  diff\_test\_cens\_cindex\_median &  time\_training\_time &  diff\_test\_cens\_Dcal\_cens \\
    & & \multicolumn{6}{c}{---------------------------------------------- Difference: CQRNN - Sequential-grid ----------------------------------------------}\\ 
    
    
   Dataset &  Number & Training time (seconds) &  Test time (seconds) &  TQMSE &  Uncensored quantile loss  &  Concordance-Index &  Censored D-Calibration \\
   
    & quantiles & (lower better) &  (lower better) & (lower better) &  (lower better)  &  (higher better) &  (lower better) \\
   
%   Uncensored quantile loss & Uncensored D-Calibration & Concordance-Index & Censored D-Calibration

\midrule
   Norm linear &           10 &                   -4.997 &                       -0.015 &                       -2.691 &                  -0.106 &                         0.001 &                    -0.013 \\
  Norm non-lin &           10 &                   -5.336 &                       -0.017 &                        0.001 &                   0.000 &                         0.001 &                    -0.008 \\
   Exponential &           10 &                   -7.528 &                       -0.026 &                       -0.404 &                  -0.004 &                         0.001 &                     0.022 \\
       Weibull &           10 &                   -7.274 &                       -0.023 &                       -0.006 &                   0.002 &                         0.000 &                     0.002 \\
       LogNorm &           10 &                   -6.145 &                       -0.018 &                        0.083 &                   0.000 &                        -0.001 &                    -0.032 \\
  Norm uniform &           10 &                   -4.853 &                       -0.015 &                        0.200 &                   0.033 &                         0.001 &                    -0.368 \\
    Norm heavy &           20 &                  -23.801 &                       -0.097 &                       -0.018 &                   0.003 &                        -0.001 &                     0.103 \\
     Norm med. &           20 &                  -24.384 &                       -0.102 &                       -0.050 &                  -0.010 &                         0.001 &                    -0.002 \\
    Norm light &           20 &                  -24.417 &                       -0.097 &                       -0.038 &                  -0.006 &                         0.000 &                    -0.106 \\
     Norm same &           20 &                  -29.910 &                       -0.125 &                       -0.685 &                  -0.062 &                         0.002 &                    -0.050 \\
 LogNorm heavy &           20 &                  -45.441 &                       -0.268 &                        0.004 &                   0.002 &                         0.001 &                    -0.008 \\
  LogNorm med. &           20 &                  -33.679 &                       -0.195 &                        0.014 &                   0.002 &                         0.000 &                    -0.034 \\
 LogNorm light &           20 &                  -45.157 &                       -0.248 &                       -0.026 &                  -0.003 &                         0.000 &                    -0.075 \\
  LogNorm same &           20 &                  -27.471 &                       -0.158 &                       -0.285 &                  -0.018 &                        -0.001 &                    -0.046 \\

\midrule
Datasets where  & & 14/14 & 14/14 & 9/14 & 8/14 & 9/14 & 11/14 \\
CQRNN is favoured  \\
\bottomrule



\end{tabular}}
\label{tab_grid_cqrnn_compare}
\caption{Performance comparison of our proposed CQRNN algorithm (alg. \ref{alg_cqrnn_loss}) with the sequential grid-based method from \cite{Neocleous2006}, which we've adapted for neural networks.
% Both optimise Portnoy's estimator, but 
For all quantile metrics CQRNN has a slight advantage (e.g. wins on 9/14 datasets in MSE). Running time for the sequential grid is significantly slower at both train and test time (and also in memory requirements). This arises from its running time scaling with, $\mathcal{O}(\text{no. quantiles})$. \tp{could delete other metric columns, keep TQMSE and put inline w text? Need parameter count}}
\end{table}

==> tables_figs_etc/table_comparison_grid_02.tex <==
\begin{table}[t]
\centering
\caption{Performance of our proposed CQRNN algorithm (algorithm \ref{alg_cqrnn_loss}) compared to the sequential grid method for NNs (algorithm \ref{alg_seq_grid}). All datasets shown -- extended version of table \ref{tab_grid_cqrnn_compare_mini}.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}
\resizebox{0.7\textwidth}{!}{\begin{tabular}{lrrrrrrr}

\toprule
   Dataset &  Number & Training time &  Test time &  Parameter & TQMSE difference  \\
  
    & quantiles & speed up &  speed up & saving &  Seq. grid $-$ CQRNN  \\
    % &&&&& Seq. grid $-$ CQRNN\\
%   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\
\midrule
   Norm linear &           10 &                    14.7$\times$ &                        11.2$\times$ &             9.2$\times$ &                         -2.691 \\
  Norm non-lin &           10 &                    12.4$\times$ &                         9.6$\times$ &             9.2$\times$ &                          0.001 \\
   Exponential &           10 &                    12.4$\times$ &                         8.0$\times$ &             9.2$\times$ &                         -0.404 \\
       Weibull &           10 &                    12.5$\times$ &                         8.7$\times$ &             9.2$\times$ &                         -0.006 \\
       LogNorm &           10 &                    12.9$\times$ &                         8.8$\times$ &             9.2$\times$ &                          0.083 \\
  Norm uniform &           10 &                    12.6$\times$ &                         8.1$\times$ &             9.2$\times$ &                          0.200 \\
    Norm heavy &           20 &                    31.0$\times$ &                        18.5$\times$ &             17.1$\times$ &                         -0.018 \\
     Norm med. &           20 &                    34.1$\times$ &                        17.9$\times$ &             17.1$\times$ &                         -0.050 \\
    Norm light &           20 &                    31.7$\times$ &                        19.2$\times$ &             17.1$\times$ &                         -0.038 \\
     Norm same &           20 &                    34.3$\times$ &                        21.2$\times$ &             17.1$\times$ &                         -0.685 \\
 LogNorm heavy &           20 &                    33.6$\times$ &                        19.9$\times$ &             17.1$\times$ &                          0.004 \\
  LogNorm med. &           20 &                    31.3$\times$ &                        13.1$\times$ &             17.1$\times$ &                          0.014 \\
 LogNorm light &           20 &                    31.3$\times$ &                        20.2$\times$ &             17.1$\times$ &                         -0.026 \\
  LogNorm same &           20 &                    29.8$\times$ &                        18.4$\times$ &             17.1$\times$ &                         -0.285 \\
\midrule
CQRNN is best:   & & 14/14 & 14/14 & 14/14 & 9/14 \\
% CQRNN is best  \\
\bottomrule

\end{tabular}}
\label{tab_grid_cqrnn_compare}
\end{table}

==> tables_figs_etc/table_comparison_grid_02_mini.tex <==
\begin{table}[t]
\centering
\caption{Performance of our proposed CQRNN algorithm (Algorithm \ref{alg_cqrnn_loss}) compared to the sequential grid method for NNs (Algorithm \ref{alg_seq_grid}). Select datsets shown -- see Table \ref{tab_grid_cqrnn_compare} for others.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}
\resizebox{0.6\textwidth}{!}{\begin{tabular}{lrrrrrrr}

\toprule
   Dataset &  Number & Training time &  Test time &  Parameter & TQMSE  \\
  
    & quantiles & speed up &  speed up & saving &  difference  \\
%   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\
\midrule
%   Norm linear &           10 &                    14.7$\times$ &                        11.2$\times$ &             9.2$\times$ &                         -2.691 \\
  Norm non-linear &           10 &                    12.4$\times$ &                         9.6$\times$ &             9.2$\times$ &                          0.001 \\
  Exponential &           10 &                    12.4$\times$ &                         8.0$\times$ &             9.2$\times$ &                         -0.404 \\
      Weibull &           10 &                    12.5$\times$ &                         8.7$\times$ &             9.2$\times$ &                         -0.006 \\
    %   LogNorm &           10 &                    12.9$\times$ &                         8.8$\times$ &             9.2$\times$ &                          0.083 \\
%   Norm uniform &           10 &                    12.6$\times$ &                         8.1$\times$ &             9.2$\times$ &                          0.200 \\
    % Norm heavy &           20 &                    31.0$\times$ &                        18.5$\times$ &             17.1$\times$ &                         -0.018 \\
    %  Norm med. &           20 &                    34.1$\times$ &                        17.9$\times$ &             17.1$\times$ &                         -0.050 \\
    % Norm light &           20 &                    31.7$\times$ &                        19.2$\times$ &             17.1$\times$ &                         -0.038 \\
    %  Norm same &           20 &                    34.3$\times$ &                        21.2$\times$ &             17.1$\times$ &                         -0.685 \\
 LogNorm heavy &           20 &                    33.6$\times$ &                        19.9$\times$ &             17.1$\times$ &                          0.004 \\
%   LogNorm med. &           20 &                    31.3$\times$ &                        13.1$\times$ &             17.1$\times$ &                          0.014 \\
 LogNorm light &           20 &                    31.3$\times$ &                        20.2$\times$ &             17.1$\times$ &                         -0.026 \\
%   LogNorm same &           20 &                    29.8$\times$ &                        18.4$\times$ &             17.1$\times$ &                         -0.285 \\
% \midrule
% CQRNN is best:   & & 14/14 & 14/14 & 14/14 & 9/14 \\
% CQRNN is best  \\
\bottomrule

\end{tabular}}
\label{tab_grid_cqrnn_compare_mini}
\end{table}

==> tables_figs_etc/table_comparison_grid_03_mini.tex <==
\begin{table}[t]
\centering
\caption{Performance of our proposed CQRNN algorithm compared to the sequential grid method for NNs. See Table \ref{tab_grid_cqrnn_compare} for results on further datasets, as well as statistical significance tests.}
% CQRNN has a slight advantage on 9/14 datasets in terms of TQMSE. 
% But the major gains are seen in improved efficiencies in train time, test time, and memory. Times refer to `wall-clock' time.}
% \resizebox{0.6\textwidth}{!}{\begin{tabular}{lrrrrrrr}

% \toprule
% %   Dataset &  Number & Training time &  Test time &  Parameter & TQMSE  \\
  
%     % & quantiles & speed up &  speed up & saving &  difference  \\
% %   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\
% \midrule
% %   Norm linear &           10 &                    14.7$\times$ &                        11.2$\times$ &             9.2$\times$ &                         -2.691 \\
%   Norm non-linear &           10 &                    12.4$\times$ &                         9.6$\times$ &             9.2$\times$ &                          0.001 \\
%   Exponential &           10 &                    12.4$\times$ &                         8.0$\times$ &             9.2$\times$ &                         -0.404 \\
%       Weibull &           10 &                    12.5$\times$ &                         8.7$\times$ &             9.2$\times$ &                         -0.006 \\
%     %   LogNorm &           10 &                    12.9$\times$ &                         8.8$\times$ &             9.2$\times$ &                          0.083 \\
% %   Norm uniform &           10 &                    12.6$\times$ &                         8.1$\times$ &             9.2$\times$ &                          0.200 \\
%     % Norm heavy &           20 &                    31.0$\times$ &                        18.5$\times$ &             17.1$\times$ &                         -0.018 \\
%     %  Norm med. &           20 &                    34.1$\times$ &                        17.9$\times$ &             17.1$\times$ &                         -0.050 \\
%     % Norm light &           20 &                    31.7$\times$ &                        19.2$\times$ &             17.1$\times$ &                         -0.038 \\
%     %  Norm same &           20 &                    34.3$\times$ &                        21.2$\times$ &             17.1$\times$ &                         -0.685 \\
%  LogNorm heavy &           20 &                    33.6$\times$ &                        19.9$\times$ &             17.1$\times$ &                          0.004 \\
% %   LogNorm med. &           20 &                    31.3$\times$ &                        13.1$\times$ &             17.1$\times$ &                          0.014 \\
%  LogNorm light &           20 &                    31.3$\times$ &                        20.2$\times$ &             17.1$\times$ &                         -0.026 \\
% %   LogNorm same &           20 &                    29.8$\times$ &                        18.4$\times$ &             17.1$\times$ &                         -0.285 \\
% % \midrule
% % CQRNN is best:   & & 14/14 & 14/14 & 14/14 & 9/14 \\
% % CQRNN is best  \\

\resizebox{0.7\textwidth}{!}{\begin{tabular}{lrrrrrrrccc}

\toprule
   Dataset &  Number & Training time &  Test time &  Parameter  & TQMSE difference \\%  & CQRNN is & Seq. grid is & No statistical \\
  
    & quantiles & speed up &  speed up & saving &  Seq. grid $-$ CQRNN  \\% &  sig. better & sig. better & significant \\
    & & & & & w/ 95\% conf. int. \\
    % & & & & \\% & 95\% conf. interval & in TQMSE? & in TQMSE? & difference \\
    % &&&&& Seq. grid $-$ CQRNN\\
%   dataset\_str &  n\_quantiles &  rel\_time\_training\_time &  rel\_time\_test\_fwdpass\_time &  paramcount\_rel &  diff\_test\_q\_metric\_selected \\

\midrule
%   Norm linear &           9 &   14.7$\times$ &   11.2$\times$ &  8.3$\times$ &          -2.189 $\pm$ 0.245 & \checkmark & & \\
 Norm non-linear &           9 &   12.4$\times$ &   9.6$\times$ &  8.3$\times$ &         -0.003 $\pm$ 0.001 \\% & \checkmark & & \\
  Exponential &           9 &   12.4$\times$ &   8.0$\times$ &  8.3$\times$ &           -0.093 $\pm$ 0.176 \\% &  & & \checkmark\\
      Weibull &           9 &   12.5$\times$ &   8.7$\times$ &  8.3$\times$ &         -0.014 $\pm$ 0.016 \\% &  & & \checkmark \\
    %   LogNorm &           9 &   12.9$\times$ &   8.8$\times$ &  8.3$\times$ &         -0.039 $\pm$ 0.028 & \checkmark & & \\
%  Norm uniform$^*$ &           9 &   12.6$\times$ &   8.1$\times$ &  8.3$\times$ &          0.175 $\pm$ 0.033 & & \checkmark  & \\
%   Norm heavy &           19 &  31.0$\times$ &        18.5$\times$ &        16.2$\times$ &           0.108 $\pm$ 0.211 & & & \checkmark\\
    % Norm med. &           19 &  34.1$\times$ &        17.9$\times$ &        16.2$\times$ &          -0.046 $\pm$ 0.004 & \checkmark & & \\
%   Norm light &           19 &  31.7$\times$ &            19.2$\times$ &     16.2$\times$ &         -0.035 $\pm$ 0.003 & \checkmark & & \\
    % Norm same &           19 &  34.3$\times$ &            21.2$\times$ &     16.2$\times$ &         -0.390 $\pm$ 0.049 & \checkmark & & \\
LogNorm heavy &           19 &  33.6$\times$ &        19.9$\times$ &        16.2$\times$ &          0.005 $\pm$ 0.001 \\% & & \checkmark &  \\
%  LogNorm med. &           19 &  31.3$\times$ &        13.1$\times$ &        16.2$\times$ &          0.019 $\pm$ 0.002 & & \checkmark &  \\
LogNorm light &           19 &  31.3$\times$ &        20.2$\times$ &        16.2$\times$ &         -0.033 $\pm$ 0.004 \\% & \checkmark & & \\
%  LogNorm same &           19 &  29.8$\times$ &        18.4$\times$ &        16.2$\times$ &         -0.371 $\pm$ 0.045 & \checkmark & & \\
% \midrule
% \midrule
\bottomrule

\end{tabular}}
\label{tab_grid_cqrnn_compare_mini}
\end{table}

==> tables_figs_etc/table_dataset_info_02_maxdef.tex <==
\begin{table}[hb]
\centering
\caption{Summary of all datasets used. See appendix \ref{sec_app_dataset_details} for further detail.}
\resizebox{0.9\textwidth}{!}{\begin{tabular}{lrrrrrcc}
\toprule
    
     \multicolumn{1}{l}{Dataset} &  \multicolumn{1}{c}{Feats} &  \multicolumn{1}{c}{Train}  &  \multicolumn{1}{c}{Test} &  Prop.  &  Max defined & Target sampling & Censoring sampling  \\
     
     & & \multicolumn{1}{c}{data} & \multicolumn{1}{c}{data} & censored & global quantile & distribution  & distribution  \\
\midrule
\multicolumn{8}{c}{\textbf{Type 1 -- Synthetic datasets with synthetic censoring}}\\
     Norm linear &        1 &      500 &    1000 &             0.20 &                       0.99 & $\mathcal{N}(2x+10,(x+1)^2)$ & $\mathcal{N}(4x+10,(0.8x+0.4)^2)$ \\
 Norm non-linear &        1 &      500 &    1000 &             0.24 &                       1.00 & $\mathcal{N}(x\sin(2x)+10,(0.5x+0.5)^2)$ & $\mathcal{N}(2x+10,2^2)$ \\
     Exponential &        1 &      500 &    1000 &             0.30 &                       0.99 & $\operatorname{Exp}(2x+4)$ & $\operatorname{Exp}(-3x+15)$ \\
         Weibull &        1 &      500 &    1000 &             0.22 &                       0.97 & $\operatorname{Weibull}(4x \sin(2(x-1))+10, 5)$ & $\operatorname{Weibull}(-3x+20, 5)$ \\
         LogNorm &        1 &      500 &    1000 &             0.21 &                       0.96 & $\operatorname{Lognorm}((x-1)^2, x^2)$ & $\mathcal{U}(0, 10)$ \\
    Norm uniform &        1 &      500 &    1000 &             0.62 &                       0.99 & $\mathcal{N}(2x \cos(2x)+13,(x^2+0.5)^2)$ & $\mathcal{U}(0, 18)$\\
      Norm heavy &        4 &     2000 &    1000 &             0.80 &                       0.75 &  \scriptnotesize $\mathcal{N}(3x_0 + x_1^2 - x_2^2 + 2\sin(x_2 x_3)+6,(x^2+0.5)^2)$ & $\mathcal{U}(0, 12)$ \\
       Norm med. &        4 &     2000 &    1000 &             0.49 &                       1.00 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 20)$ \\
      Norm light &        4 &     2000 &    1000 &             0.25 &                       1.00 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 40)$ \\
       Norm same &        4 &     2000 &    1000 &             0.50 &                       0.98 & --- \raisebox{-0.5ex}{''} --- & Equal to target dist.  \\
   LogNorm heavy &        8 &     4000 &    1000 &             0.75 &                       0.47 & $\operatorname{Lognorm}(\sum_i^8 \beta_i x_i, 1)/10$ & $\mathcal{U}(0, 0.4)$ \\
    LogNorm med. &        8 &     4000 &    1000 &             0.52 &                       0.73 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 1.0)$\\
   LogNorm light &        8 &     4000 &    1000 &             0.23 &                       0.94 & --- \raisebox{-0.5ex}{''} --- & $\mathcal{U}(0, 3.5)$\\
    LogNorm same &        8 &     4000 &    1000 &             0.50 &                       0.99 & --- \raisebox{-0.5ex}{''} --- & Equal to target dist.  \\
    
        \\ \multicolumn{8}{c}{ \textbf{Type 2 -- Real datasets with synthetic censoring} }\\
         
         Housing &        8 &    16512 &    4128 &             0.50 &                       0.90 & Real & $\mathcal{U}(0, c_1)$ \\
         Protein &        9 &    36584 &    9146 &             0.44 &                       0.90 & Real & $\mathcal{U}(0, c_2)$\\
            Wine &       11 &     5197 &    1300 &             0.69 &                       0.90 & Real & $\mathcal{U}(0, c_3)$\\
             PHM &       21 &    36734 &    9184 &             0.52 &                       0.90 & Real & $\mathcal{U}(0, c_4)$\\
       SurvMNIST &        28$\times$28 &    48000 &   12000 &             0.53 &                       0.90 & One Gamma dist. per MNIST class & $\mathcal{U}(0, c_5)$ \\
        
        \\ \multicolumn{8}{c}{ \textbf{Type 3 -- Real datasets with real censoring} }\\
        METABRIC &        9 &     1523 &     381 &             0.42 &                       0.99 & Real & Real \\
            WHAS &        6 &     1310 &     328 &             0.57 &                       0.64 & Real & Real\\
         SUPPORT &       14 &     7098 &    1775 &             0.32 &                       0.76 & Real & Real\\
            GBSG &        7 &     1785 &     447 &             0.42 &                       0.63 & Real & Real\\
       TMBImmuno &        3 &     1328 &     332 &             0.49 &                       0.80 & Real & Real\\
       BreastMSK &        5 &     1467 &     367 &             0.77 &                       0.61 & Real & Real\\
          LGGGBM &        5 &      510 &     128 &             0.60 &                       0.89 & Real & Real\\
\bottomrule
\end{tabular}}
\label{tab_dataset_info}
\end{table}


